Testing Convex Truncation

We study the basic statistical problem of testing whether normally distributed $n$-dimensional data has been truncated, i.e. altered by only retaining points that lie in some unknown truncation set $S \subseteq \mathbb{R}^n$. As our main algorithmic results, (1) We give a computationally efficient $O(n)$-sample algorithm that can distinguish the standard normal distribution $N(0,I_n)$ from $N(0,I_n)$ conditioned on an unknown and arbitrary convex set $S$. (2) We give a different computationally efficient $O(n)$-sample algorithm that can distinguish $N(0,I_n)$ from $N(0,I_n)$ conditioned on an unknown and arbitrary mixture of symmetric convex sets. These results stand in sharp contrast with known results for learning or testing convex bodies with respect to the normal distribution or learning convex-truncated normal distributions, where state-of-the-art algorithms require essentially $n^{\sqrt{n}}$ samples. An easy argument shows that no finite number of samples suffices to distinguish $N(0,I_n)$ from an unknown and arbitrary mixture of general (not necessarily symmetric) convex sets, so no common generalization of results (1) and (2) above is possible. We also prove that any algorithm (computationally efficient or otherwise) that can distinguish $N(0,I_n)$ from $N(0,I_n)$ conditioned on an unknown symmetric convex set must use $\Omega(n)$ samples. This shows that the sample complexity of each of our algorithms is optimal up to a constant factor.

==> sections/Anindya_s_folder/algorithms.tex <==
%!TEX root = ../distinguishing-writeup.tex


\section{Glorious Algorithmic Results}


\input{csc-sets}

\input{csc-mixtures}

\input{general-convex}

\input{halfspaces}

==> sections/Anindya_s_folder/csc-mixtures.tex <==
%!TEX root = ../distinguishing-writeup.tex

\subsection{A $\tilde{O}(n/\eps^2)$-sample algorithm for mixtures of symmetric convex sets - PROFESSOR DE}


\begin{theorem} \label{thm:mix}
There is an algorithm with the following performance guarantee:  given any $\eps > 0$ and access to independent samples from any unknown distribution ${\cal D} \in \Mix$, the algorithm uses $\tilde{O}(n)/\eps^2$ samples, and


\begin{enumerate}

\item If ${\cal D}=N(0,I_n)$, then with probability at least $9/10$ the algorithm outputs ``un-truncated'';

\item If $\dtv({\cal D},N(0,I_n)) \geq \eps$, then with probability at least $9/10$ the algorithm outputs ``truncated.''

\end{enumerate}

\end{theorem}


==> sections/Anindya_s_folder/csc-sets.tex <==
%!TEX root = ../distinguishing-writeup.tex

\subsection{A $\tilde{O}(n/\eps^2)$-sample algorithm for symmetric convex sets - PROFESSOR DE}

%{\shivam{Grabbed token for this}}

\

\begin{theorem} \label{thm:symmetric}
There is an algorithm with the following performance guarantee:  given any $\eps > 0$ and access to independent samples from any unknown distribution ${\cal D} \in \Psymm$, the algorithm uses $\tilde{O}(n)/\eps^2$ samples, and

\begin{enumerate}

\item If ${\cal D}=N(0,I_n)$, then with probability at least $9/10$ the algorithm outputs ``un-truncated'';

\item If $\dtv({\cal D},N(0,I_n)) \geq \eps$, then with probability at least $9/10$ the algorithm outputs ``truncated.''

\end{enumerate}

\end{theorem}


We begin  by describing the algorithm for Theorem~\ref{thm:symmetric} followed by its analysis. 

\begin{enumerate}
\item Sample $T$ points $\bx^{(1)}, \ldots, \bx^{(T)}$ 
from $\cal D$ where $T = \tilde{O}(n)/\epsilon^2$. 
\item If there exists $1 \le i \le T$ such that $\Vert \bx^{(i)} \Vert_2^2 \ge n + 2 \sqrt{n \log (n/\epsilon)}$, then output ``truncated". 
\item Otherwise, compute $\langle \Vert x \Vert_2^2 \rangle := \frac{1}{T} \cdot (\sum_{i=1}^T \Vert \bx^{(i)} \Vert_2^2$. 
\end{enumerate}


To analyze this algorithm, we will need the following lemmas. 
\begin{lemma}
If ${\cal D} = N(0, I_n)$, then with probability $0.99$, for $T$ points $\bx^{(1)}, \ldots, \bx^{(T)}$  sampled from ${\cal D}$, each point $\bx^{(i)}$ satisfies $\Vert \bx^{(i)} \Vert_2^2 \ge n + 2 \sqrt{n \log (n/\epsilon)}$. 
\end{lemma}
\begin{proof} 
When $\bx \sim N(0, I_n)$, then $\Vert \bx \Vert_2^2$ follows $\chi^2(0,n)$. The claim now follows immediately from Fact ... 
\end{proof} 


We next state the following important claim. 
\begin{claim}~\label{clm:csc-gapexp}
Let $K \subseteq \mathbb{R}^n$ be a centrally symmetric convex set. Define ${\cal D} = N(0,I_n)_K$. Then, 
\[
\mathbf{E}_{\bx \sim {\cal D}} [\Vert \bx \Vert_2^2] = n - \frac{I(K)}{\gamma(K)}. 
\]
\end{claim} 
\begin{proof}
Let $K(\cdot)$ be used as the indicator function of the set $K$. By definition of $I(K)$, we have 
\[
\mathbf{E}_{\bx \sim N(0,I_n)} [K(\bx) \cdot (n-\Vert \bx \Vert_2^2)] = I(K). 
\]
As $K(\cdot)$ is a $0/1$ valued function, the left hand side of the above equation can be rewritten as 
\[
\gamma(K) \cdot \mathbf{E}_{\bx \sim N(0,I_n)_K} [(n-\Vert \bx \Vert_2^2)]  = I(K). 
\]
This finishes the proof. 
\end{proof} 

We now recall the following \Poincare-type inequality from \cite{DNS21}. 
\begin{lemma} ~\label{lem:poincare}
If $K \subseteq \mathbb{R}^n$, then $I(K) \ge \Theta(\Var(K))$. 
\end{lemma}

Combining Lemma~\ref{lem:poincare} and Claim~\ref{clm:csc-gapexp}, we have the following corollary.
\begin{corollary}
Let $K$ be symmetric convex set such that $\gamma(K) \le 1-\epsilon$. Then, for ${\cal D} = N(0,I_n)_K$, 
$\mathbf{E}_{\bx \sim {\cal D}} [\Vert \bx \Vert_2^2] \le n- \Theta(\epsilon)$. 
\end{corollary} 
\begin{proof}
By Claim~\ref{clm:csc-gapexp} and Lemma~\ref{lem:poincare}, we have 
\[
\mathbf{E}_{\bx \sim {\cal D}} [\Vert \bx \Vert_2^2]  = n-\frac{I(K)}{\gamma(K)} \le n - \frac{\Theta(\Var(K))}{\gamma(K)}. 
\]
Since $\gamma(K) \leq 1-\epsilon$, it follows that $\Var(K)/\gamma(K) \ge \epsilon$. This finishes the proof. 
\end{proof}

\begin{proofof}{Theorem~\ref{thm:symmetric}} 
If ${\cal D} = N(0,I_n)$, then with 

\end{proofof}

\violet{
\noindent {\bf Sketch:}
See  \href{https://www.dropbox.com/home/Anindya-Shivam-distinguishing-satisfying-assignments/our-notes?preview=note.pdf}{Section 3 of our note.pdf file} and also 
\href{https://www.dropbox.com/home/Anindya-Shivam-distinguishing-satisfying-assignments/our-notes?preview=convex.pdf}{Section 1.1 of our convex.pdf file}  for rough early notes on the approach. 

The high level description of the tester is that it is somewhat analogous to the algorithm of Theorem~4 (the uniformity testing result) of \cite{RubinfeldS09}.  The algorithm draws its sample of $\tilde{O}(n)$ samples and checks to make sure that none of them have $|\|x\| - \sqrt{n}|$ larger than $c\sqrt{\log n}$ or so --- if any of them lie outside that shell the algorithm outputs ``not Gaussian,'' and otherwise it proceeds to the ``real algorithm'' (estimating the total convex influence, etc).  The high level idea is that by virtue of doing this checking/conditioning, if we get to the ``real algorithm'' then each of its samples $\bx$ has $\|\bx\|$ drawn from an interval of width $c\sqrt{\log n}$ around $\sqrt{n}$, so each sample has $\|\bx\|^2$ drawn from an interval of width $\sqrt{n \log n}$ and hence we have $\Var[\|\bx\|^2] \leq n \log n.$

TODO: go carefully through the analysis based on convex influence / Poincare and work out details of all cases. If $\vol(K)$ is not too tiny, say at least $0.01$, then I think we are fine by our old convex influence type / Poincare analysis (note the volume can't be more than $1-\eps$ by assumption). If $\vol(K)$ is very tiny then there are a few possibilities. If $\rinn$ is at least $1/2$ (as would be the case e.g. with a small-volume ball as $K$) then we use the fact that $\E[\|\bx\|^2]$ is $n - \TInf(K)/\gamma(K)=n-\Omega(\rinn)\leq n-\Theta(1)$ to get the desired gap in the means. If $\rinn < 1/2$ then the entire body is contained in a slab of width at most $1$ and this also gives the desired gap in the means (even if the $n-1$ other coordinates were totally unconstrained $\E[\|\bx\|^2]$ would be at most $n - 1 + 1/4$).
}

==> sections/Anindya_s_folder/general-convex.tex <==
%!TEX root = ../distinguishing-writeup.tex

\subsection{A $\tilde{O}(n/\eps^2)$-sample algorithm for general convex sets - SHIVAM}

\begin{theorem} \label{thm:convex}
There is an algorithm with the following performance guarantee:  given any $\eps > 0$ and access to independent samples from any unknown distribution ${\cal D} \in \Pconv$, the algorithm uses $\tilde{O}(n)/\eps^2$ samples, and

\begin{enumerate}

\item If ${\cal D}=N(0,I_n)$, then with probability at least $9/10$ the algorithm outputs ``un-truncated'';

\item If $\dtv({\cal D},N(0,I_n)) \geq \eps$, then with probability at least $9/10$ the algorithm outputs ``truncated.''

\end{enumerate}

\end{theorem}

\violet{
\noindent {\bf Sketch:}


See \href{https://www.dropbox.com/home/Anindya-Shivam-distinguishing-satisfying-assignments/our-notes?preview=convex.pdf}{our convex.pdf file} for a sketch of the case in which $\vol(K) \geq 0.1$.

TODO:  Think about how to handle small volume general convex sets,
}




==> sections/Anindya_s_folder/halfspaces.tex <==
%!TEX root = ../distinguishing-writeup.tex

\subsection{A $\tilde{O}(\sqrt{n}/\eps^2)$-sample algorithm for LTFs - SHIVAM}
\label{subsec:halfspaces}

\red{TODO: Say that this is essentially Dicker's estimator? Also have to mention the Xi-Chen result.}


\begin{algorithm}
\caption{Distinguisher for LTFs}
\label{alg:halfspaces}
\vspace{0.5em}
\textbf{Input:} $\calD\in\Pltf$, $\eps > 0$\\[0.5em]
\textbf{Output:} ``Un-truncated'' or  ``truncated''

\ 

\LTF$(\calD, \epsilon)$:
\begin{enumerate}
    \item 
\end{enumerate}

\end{algorithm}

\begin{theorem} \label{thm:LTF}
There is an algorithm \LTF\ (cf. \Cref{alg:halfspaces}) with the following performance guarantee:  given any $\eps > 0$ and access to independent samples from any unknown distribution ${\cal D} \in \Pltf$, the algorithm uses $\tilde{O}(\sqrt{n})/\eps^2$ samples, and

\begin{enumerate}

\item If ${\cal D}=\calN(0,1)^n$, then with probability at least $9/10$ the algorithm outputs ``un-truncated'';

\item If $\dtv\pbra{{\cal D}, \calN(0,1)^n} \geq \eps$, then with probability at least $9/10$ the algorithm outputs ``truncated.''

\end{enumerate}

\end{theorem}

\begin{proof}
	
	
	
	
\end{proof}

%\violet{
%\noindent {\bf Sketch:}
%See \href{https://www.dropbox.com/home/Anindya-Shivam-distinguishing-satisfying-assignments/our-notes?preview=convex.pdf}{Section~2.1.1 of our convex.pdf file} for an analysis of the Dicker estimator in the $\vol(K)=1/2$ (i.e. origin-centered LTF) case. We  need  to  also mention the Xi  Chen result.
%}



==> sections/Anindya_s_folder/intro.tex <==
%!TEX root = distinguishing-writeup.tex

\section{Glorious Introduction}
\label{sec:intro}

Introduce the general problem: we study the problem of determining whether an unknown distribution, that you have sample access to, is a high-dimensional standard normal distribution versus a truncated normal distribution. In this level of generality the problem is impossible for two reasons: first is simply  that if the truncation discards  only  a negligible amount of mass then of course it's undetectable. So we require our truncations to produce a distribution with significant variation distance  from  the original $N(0,I_n)$ distribution, i.e.  to discard a nonnegligible amount of mass. Second  reason is that if no  restrictions are  put on what kind of  truncations may be performed, then easily seen to be impossible.(Example of). So  we must consider restricted types of allowed truncations.

Our focus is on the setting when the truncations are given by convex sets, and variants (our symmetric convex sets, mixtures of CSC distributions, and so on).

\subsection{Background and motivation}

\begin{itemize}

\item Determining whether or not a null hypothesis holds is of course a very basic paradigm of a question in statistics.\rnote{I don't know what I'm talking about here.}

\item Connect it with the ``learning Gaussians from truncated samples'' \cite{DGTZ} line of work and other problems of truncated statistics. Arguably an even more basic first thing to understand than  learning  from truncated samples is algorithms and lower bounds on determining whether any statistically significant truncation has taken place at all.  Convex sets and  their generalizations that we consider are a very basic type of truncation (maybe explicitly considered in \cite{DGTZ}? Check that paper)\snote{See also \cite{Kontonis2019} where they explicitly consider estimating the mean and covariance of a Gaussian from samples from a convex truncation?}  

\item Has something of the spirit of property testing type questions of the sort ``given a distribution that is promised to be of type X, is it the uniform distribution''?  Mention papers that e.g. ask and answer this question where type X is ``monotone distributions over $\{1,\dots,N\}$''; where type X is ``monotone distributions over $\zo^n$'' (\cite{RubinfeldS09}); and so on.

\item Also has connections to well studied problems of learning convex sets (throw in some cites including \cite{KOS:08}) and testing convex sets (throw in cites including \cite{CFSS17}).

\end{itemize}

\subsection{Our results}

\subsubsection{Efficient distinguishing algorithms}
We start by describing our most basic distinguishing result, which is an algorithm for symmetric convex sets (we will soon generalize this result in two different ways).  In the following informal theorem statement, given a set $K \subseteq \R^n$, we write $N(0,I_n)|_K$ to denote the standard Normal distribution conditioned on $K$.

\begin{theorem} \label{thm:symmetric-convex}
[Symmetric convex truncations, informal theorem statement]
There is an algorithm $\Asymm$ which uses $\tilde{O}(n/\eps^2)$ samples, runs in $\poly(n,1/\eps)$ time, and distinguishes between the standard $N(0,I_n)$ distribution and any distribution ${\cal D}=N(0,I_n)|_S$ where $S \subset \R^n$ is any symmetric convex set such that $\dtv(N(0,I_n),N(0,I_n)|_S) \geq \eps.$
\end{theorem}

\emph{(Few words about the algorithm - what it estimates, but not going into the same level of detail as in the next section)}
By extending the analysis of the algorithm of \Cref{thm:symmetric-convex} we are able to show that the same algorithm in fact succeeds for a broader class of truncations, namely truncation by any mixture of symmetric convex distributions:


\begin{theorem} \label{thm:symmetric-convex-mixture}
[Mixtures of symmetric convex truncations, informal theorem statement]
The algorithm $\Asymm$ uses $\tilde{O}(n/\eps^2)$ samples, runs in $\poly(n,1/\eps)$ time, and distinguishes between the standard $N(0,I_n)$ distribution and any distribution ${\cal D}$ which is a normal distribution conditioned on a mixture of symmetric convex sets such that $\dtv(N(0,I_n),{\cal D}) \geq \eps.$
\end{theorem}

It's not hard to show that the algorithm of \Cref{thm:symmetric-convex} does not succeed for truncation by general (non-symmetric) convex sets.  We show that a different algorithm can handle general convex sets:

\begin{theorem} \label{thm:general-convex}
[General convex truncations, informal theorem statement]
There is an algorithm $\Aconv$ which uses $\tilde{O}(n/\eps^2)$ samples, runs in $\poly(n,1/\eps)$ time, and distinguishes between the standard $N(0,I_n)$ distribution and any distribution ${\cal D}=N(0,I_n)|_S$ where $S \subset \R^n$ is any convex set such that $\dtv(N(0,I_n),N(0,I_n)|_S) \geq \eps.$
\end{theorem}

It is tempting to wonder about a common generalization, to mixtures of general convex sets, but it is impossible to have any upper bound on the sample complexity for that problem. (Forward reference to a brief appendix with this.

Finally, we also give a different and more efficient algorithm for the special case in which the truncation set is the simplest possible convex set, namely a halfspace:

\begin{theorem} \label{thm:halfspace}
[Halfspace truncations, informal theorem statement]
There is an algorithm $\Ahalf$ which uses $\tilde{O}(\sqrt{n}/\eps^2)$ samples, runs in $\poly(n,1/\eps)$ time, and distinguishes between the standard $N(0,I_n)$ distribution and any distribution ${\cal D}$ which is a normal distribution conditioned on a halfspace such that $\dtv(N(0,I_n),{\cal D}) \geq \eps.$
\end{theorem}


\subsubsection{Information-theoretic lower bounds}

We give an $\Omega(\sqrt{n})$ lower bound for CSC bodies that are intersections of two  halfspaces.  We also show that the same lower bound holds for a single (non-axis-aligned) halfspace. Our most technically involved lower bound is an $\Omega(n)$ lower bound for mixtures of CSC's. 

\emph{(Give informal theorem statements in this section.)}

\subsection{Techniques}

\noindent {\bf Upper bound techniques.}
To build intuition we first consider the case of a single CSC body.  It is easy to see that draws from ${\cal N}(0,I_n)|_K$ will on average have a smaller squared 2-norm that draws from ${\cal N}(0,I_n)$, so it is natural to try to base a test off of this.  

To make this rough idea precise, we use the notion of \emph{total convex influence} from \cite{DNSinfluence22}. In particular, we use a version of Poincare's inequality for the convex influence notion to show that if a symmetric convex set $K$ is such that $N(0,I_n)|_K$ has noticeable statistical distance from $N(0,I_n)$, then a distinguisher based on the squared length of the observed draws can succeed with linear sample complexity.  With some additional technical work in the analysis this same tester works for mixtures of CSC $N(0,I_n)|_K$'s.

The length-based tester sketched above will not succeed for general (non-symmetric) convex sets, since $\E_{\bx \sim N(0,I_n)|_K}[\|x\|]$ can be larger than $\E_{\bx \sim N(0,I_n)}[\|x\|]$ if $K$ is an arbitrary convex set.  For the class of general convex sets we borrow an idea from \cite{DS21colt} and perform a case analysis based on whether or not the set $K$ contains a reasonably large origin-centered ball.\rnote{Actually, let's discuss how we will handle general convex sets of arbitrary volume - I am not sure I remember our reasoning for the case of arbitrary volume. 

First, suppose that the convex set $K$ has volume at least $0.1$. Then if $K$ does not contain a radius-1 origin-centered ball, $K$ must have Gaussian center-of-mass far from $0^n$; our tester detects this and so I think we're okay for sets of volume at least $0.1$.

So, suppose that the convex set has small volume (less than $0.1$).   There are two possibilities: one is that it contains a radius-1 origin-centered ball and the other is that it does not. If it contains a radius-1 origin-centered ball then we can use our Poincare and we are okay. If it does not contain a radius-1 origin-centered ball (for example, this would be the case if it is lower-dimensional and has Gaussian volume 0),

}

Finally, we use a more efficient tester for the special case of halfspaces to get an improved $O(\sqrt{n})$ bound for this case.

\medskip

\noindent {\bf Lower bound techniques.}  For both single (non-axis-aligned) halfspace and ``slabs'' (symmetric convex sets that are the intersection of two halfspaces), the key ingredient in our analysis is a recent bound due to Devroye et al on the total variation distance between two Gaussians.   

Our most technically involved and quantitatively strongest lower bound is for mixtures of CSC $K$'s.  We first show that $N(0,I_n)$ is indistinguishable, given $cn$ samples, from $N(0,(1-\delta)I_n)$ for a suitable $\delta$. Next, we show that $N(0,(1-\delta)I_n)$ can be very accurately approximated (to variation distance $2^{-\Theta(n)}$) by a mixture ${\cal M}$ of $N(0,I_n)|_K$ distributions where each $K$ is a ball intersected with an $n-1$-dimensional subspace. (The subspaces are Haar uniform and the radii of the balls are carefully selected.) Finally, we adapt an idea from \cite{RubinfeldS09} and observe that $\sqrt{T}$ samples from ${\cal M}$ are indistinguishable from $\sqrt{T}$ samples from ${\cal D}$ where ${\cal D}$ is a subsampled version of the mixture ${\cal M}$ (a uniform mixture of $T$ distributions sampled from the mixture). Given this a simple argument shows that ${\cal D}$ is both indistinguishable from $N(0,I_n)$ and statistically far from $N(0,I_n)$ (in fact the total variation distance is 1).






==> sections/Anindya_s_folder/lb-halfspaces.tex <==
%!TEX root = ../distinguishing-writeup.tex

\subsection{A $\tilde{\Omega}(\sqrt{n})$ lower bound for halfspaces} \label{sec:halfspace-lb}

Our first lower bound, \Cref{thm:lb-ltf}, shows that $\Omega(\sqrt{n}/\log n)$ samples are needed to distinguish $N(0,I_n)$ from $N(0,I_n)|_K$ where $K$ is an unknown halfspace whose separating hyperplane passes through the origin. 
Some of the ideas in this lower bound will recur in our lower bound for symmetric ``slabs'' (intersections of two parallel halfspaces) given in \Cref{sec:symmetric-lb}, but by taking advantage of the fact that origin-centered halfspaces are odd functions, we can sidestep some aspects of the argument that arise for slabs; hence we give a self-contained proof for halfspaces below.

\begin{theorem} \label{thm:lb-ltf}
Let $A$ be any algorithm which is given access to samples from an unknown distribution ${\cal D}$ over $\R^n$ and has the following performance guarantee:

\begin{enumerate}

\item If ${\cal D}=N(0,I_n)$, then with probability at least $2/3$ the algorithm outputs ``un-truncated'';

\item If ${\cal D}=N(0,I_n)|_K$ where $K$ is an unknown zero-threshold LTF, then with probability at least $2/3$ the algorithm outputs ``truncated.''

\end{enumerate}
Then $A$ must use at least $\Omega(\sqrt{n}/\log n)$ samples from ${\cal D}$.
\end{theorem}

\begin{proof}
We consider two different distributions, ${\cal D}_1$ and ${\cal D}_2$, each of which is a distribution over sequences of $m$  points in $\R^n$.

\begin{enumerate}

\item A draw of $\overline{\bx}=(\bx^1,\dots,\bx^m)$ from ${\cal D}_1$  is obtained by having each $\bx^i \in \R^n$ be distributed independently according to $N(0,I_n)$.

\item A draw from ${\cal D}_2$ is obtained by independently drawing $\bg,\bg^1,\dots,\bg^m$ from  $N(0,I_n)$ and outputting $(\sign(\bg \cdot \bg^1) \bg^1, \dots, \sign(\bg\cdot \bg^m) \bg^m).$
\end{enumerate}

Observe that a draw from ${\cal D}_2$ is distributed as a sample of $m$  independent draws from $N(0,I_n)|_{\bK}$ where $\bK=\{x \in \R^n: \bg \cdot x \geq 0\}$ is a random zero-threshold LTF defined by a normal vector $\bg$ that is drawn from $N(0,I_n)$ (here is where we are using that any zero-threshold LTF is an odd function). Thus to prove \Cref{thm:lb-ltf} it suffices to show that any algorithm that determines  (with correctness probability at least $2/3$) whether an $m$-element sample came from ${\cal D}_1$ or ${\cal D}_2$ must have $m = \Omega(\sqrt{n}/\log n).$ This is an immediate consequence of the following claim: 

\begin{claim}
\label{claim:dtvhalfspace}
There is a universal constant $c>0$ such that for $m = c \sqrt{n}/\log n$, we have 
$\dtv({\cal D}_1,{\cal D}_2) \leq 0.1.$
\end{claim}

\medskip
\noindent \emph{Proof of \Cref{claim:dtvhalfspace}.}
We first observe that a draw $(\bx^1,\dots,\bx^m) \sim {\cal D}_1$ is distributed identically to $(\bu_1 \bx^1,\dots,
\bu_m \bx^m)$ where each $\bu_i$ is an independent uniform $\bits$ random variable. Next, we observe that
\begin{align} 
\dtv({\cal D}_1,{\cal D}_2) &=
\dtv((\bu_1 \bx^1,\dots,
\bu_m \bx^m),(\sign(\bg \cdot \bg^1) \bg^1, \dots, \sign(\bg\cdot \bg^m) \bg^m))\nonumber \\
&\leq\dtv((\bu_1,\dots,\bu_m),(\sign(\bg \cdot \bg^1),\dots,\sign(\bg \cdot \bg^m))) 
\tag{coupling $\overline{\bx}$ and $\overline{\bg}=(\bg^1,\dots,\bg^m)$} \nonumber
\end{align}
where $\bu=(\bu_1,\dots,\bu_m)$ is uniform over $\bits^m$. So it remains to bound the variation distance between the two $m$-bit strings $\bu$ and $(\sign(\bg \cdot \bg^1),\dots,\sign(\bg \cdot \bg^m)).$ We may view a uniform $\bu \sim \bits^m$ as being distributed according to $(\sign(\bg \cdot e^1),\dots,\sign(\bg \cdot e^m))$, so our  goal is to show that

\begin{equation} 
\label{eq:humphrey}
\dtv((\sign(\bg \cdot e^1),\dots,\sign(\bg \cdot e^m)),(\sign(\bg \cdot \bg^1),\dots,\sign(\bg \cdot \bg^m))) \leq 0.1.
\end{equation} 

We say that a specific outcome $(g^1,\dots,g^m) \in (\R^n)^m$ of $(\bg^1,\dots,\bg^m) \sim (N(0,I_n))^m$ is \emph{bad} if there is a pair $i\neq j$ such that the normalized inner product ${\frac {|g^i \cdot g^j|}{\|g^i\| \cdot \|g^j\|}}$ is greater than $C\sqrt{{\frac {\log n}n}}$, and otherwise we say that $(g^1,\dots,g^m)$ is \emph{good}. Intuitively, the tuple $(g^1,\dots,g^m)$ is bad if the $m$ vectors $g^1,\dots,g^m$ are not ``pairwise nearly orthogonal''; as we now show, this is very unlikely to happen.
Fix any $1 \leq i \neq j \leq m$; we have that ${\frac {\bg^i}{\|\bg^i\|}}$ and ${\frac {\bg^j}{\|\bg^j\|}}$ are independent uniform vectors on the $n$-dimensional unit sphere $\mathbb{S}^{n-1}$, and so the distribution of  ${\frac {|\bg^i \cdot \bg^j|}{\|\bg^i\| \cdot \|\bg^j\|}} = \left| {\frac {\bg^i}{\|\bg^i\|}} \cdot {\frac {\bg^j}{\|\bg^j\|}}\right|$ is
the same as the distribution of $|\bv_1|$ for a uniform random unit vector $\bv \sim \mathbb{S}^{n-1}$. It is well known (see e.g. \red{(cite)}) that $\Pr_{\bv \sim \mathbb{S}^{n-1}}[|\bv_1| > C \sqrt{\log(n)/n}]$ is at most $1/n^2$ for a suitable choice of the absolute constant $C$.  Thus by a union bound over all $m^2 = o(n)$ many pairs $i \neq j$, we have that 
\[
\Pr[(\bg^1,\dots,\bg^m)\text{~is bad}]\leq {\frac {m^2}{n^2}}<0.05.
\]

Hence to establish (\ref{eq:humphrey}) (and hence \Cref{claim:dtvhalfspace} and \Cref{thm:lb-ltf}) it suffices to prove the following:

\begin{claim} 
\label{claim:hubert}
Fix a good $(g^1,\dots,g^m) \in (\R^n)^m$, where $m = c\sqrt{n}/\log n$.
Then for $\bg \sim N(0,I_n)$ we have that
\begin{equation} \label{eq:mansfield-park}
\dtv((\sign(e^1 \cdot \bg),\dots,\sign(e^m \cdot \bg)),(\sign(g^1 \cdot \bg),\dots,\sign(g^m \cdot \bg))) \leq 0.05.
\end{equation}
\end{claim}
To prove \Cref{claim:hubert} we first observe that (\ref{eq:mansfield-park}) is equivalent to
\begin{equation}\label{eq:pride-and-prejudice}
\dtv((\sign(e^1 \cdot \bg),\dots,\sign(e^m \cdot \bg)),(\sign(g'^1 \cdot \bg),\dots,\sign(g'^m \cdot \bg))) \leq 0.05
\end{equation} 
where we define $g'^i := {\frac {g^i}{\|g^i\|}}$ to be $g^i$ normalized to unit length. Next we recall a recent upper bound on the total variation distance between $n$-dimensional Gaussians due to Devroye, Mehrabian and Reddad:

\begin{theorem} 
[Theorem~1.1 of \cite{DMR20}]  \label{thm:DMR20}
Let $\Sigma_1,\Sigma_2$ be two $m \times m$ positive definite covariance matrices and let $\lambda_1,\dots,\lambda_m$ be the eigenvalues of $\Sigma_1^{-1} \Sigma_2 - I_m$. Then
\[
\dtv(N(0^m,\Sigma_1),N(0^m,\Sigma_2)) \leq {\frac 3 2} \cdot \min\left\{1,\sqrt{\lambda_1^2 + \cdots + \lambda_m^2}\right\} 
\]
\end{theorem}
To apply \Cref{thm:DMR20} we take $\Sigma_1$ to be the identity matrix $I_m$ and $\Sigma_2$ to be the $m \times m$ matrix whose $(i,j)$ entry is $g'^i \cdot g'^j$, so a draw from $N(0,\Sigma_1)$ is distributed as $(e_1 \cdot \bg,\dots,e_m \cdot \bg)$ and a draw from $N(0,\Sigma_2)$ is distributed as
$(g'^1 \cdot \bg,\dots,g'^m \cdot \bg).$  Applying the data processing inequality for total variation distance (see e.g. Proposition~B.1 of \cite{DDOST13}\rnote{Is there a less ridiculous citation for this? Gautam Kamath cites  Proposition~B.1 of \cite{DDOST13} in his thesis, but there must be more reputable sources}), it follows that the LHS of (\ref{eq:pride-and-prejudice}) is at most $\dtv(N(0^m,\Sigma_1),N(0^m,\Sigma_2))$; we proceed to upper bound the RHS of \Cref{thm:DMR20}.

Let $A$ denote the matrix $\Sigma_1^{-1}\Sigma_2 - I_m$, so $\lambda_1^2,\dots,\lambda_m^2$ are the eigenvalues of $A^2$  and we have $\sqrt{\lambda_1^2 + \cdots + \lambda_m^2} = \sqrt{\tr(A^2))}.$
%(since the sum of eigenvalues of $A^2$ is the trace of $A^2$).
Since each $g'^i$ is a unit vector the matrix $A$ has zero entries on the diagonal, and $A$ has off-diagonal entries that are each at most $C \sqrt{{\frac {\log n} n}}$ in magnitude (because $(g^1,\dots,g^m)$ is good). Hence any diagonal element of $A^2$ is at most ${\frac {C^2 m \log n}{n}}$ in magnitude, and consequently $\tr(A^2) \leq {\frac {C^2 m^2  \log n}{n}}$, which is at most ${\frac 1 {900}}$ for a suitable choice of $m = \Theta(\sqrt{n/\log n}).$ Having $\tr(A^2) \leq {\frac 1 {900}}$ gives that ${\frac 3 2} \cdot \min\left\{1,\sqrt{\lambda_1^2 + \cdots + \lambda_m^2}\right\} \leq 0.05$ as required, and the proofs of \Cref{claim:hubert}, \Cref{claim:dtvhalfspace} and \Cref{thm:lb-ltf} are complete.
\end{proof}

%\href{https://arxiv.org/abs/1810.08693}{the Devroye et al paper}


==> sections/Anindya_s_folder/lb-mixtures.tex <==
%!TEX root = ../distinguishing-writeup.tex

\subsection{A $\tilde{\Omega}(n)$-sample lower bound for mixtures of symmetric convex sets - TBD}

{\shivam{Grabbed token for this}}

\

Our most involved lower bound shows that $\Omega(n)$ samples are needed to distinguish $N(0,I_n)$ from an unknown distribution in $\Mix$ even if the distribution in $\Mix$ is guaranteed to have variation distance 1 (the largest possible value) from ${\cal N}(0,I_n)$.

\begin{theorem} \label{thm:lb-mixsymm}
Let $A$ be any algorithm which is given access to samples from an unknown distribution ${\cal D}$ and has the following performance guarantee:

\begin{enumerate}

\item If ${\cal D}=N(0,I_n)$, then with probability at least $9/10$ the algorithm outputs ``un-truncated'';

\item If ${\cal D} \in \Mix$ and has $\dtv({\cal D},N(0,1)|_K)=1$ then with probability at least $9/10$ the algorithm outputs ``truncated.''

\end{enumerate}
Then $A$ must use at least $\Omega(n)$ samples from ${\cal D}$.
\end{theorem}
\violet{
{\bf Sketch:}
See \href{https://www.dropbox.com/home/Anindya-Shivam-distinguishing-satisfying-assignments/our-notes?preview=Note-Mar-30-2022.pdf}{p. 3 and 4 of these notes} for the stuff analyzing squared Hellinger distance to show that $N(0,(1-\delta)I_n)$ and $N(0,I_n)$ are $1/\delta$-sample-indistinguishable. See \href{https://www.dropbox.com/home/Anindya-Shivam-distinguishing-satisfying-assignments/our-notes?preview=RS-style-lower-bound-for-Gaussian.pdf}{p. 1--5 or so of these notes} for the stuff with integrals on how to give a high accuracy approximation of $N(0,(1-\delta)I_n)$ by balls intersected with $(n-1)$-dimensional subspaces.

}



==> sections/Anindya_s_folder/lb-slabs.tex <==
%!TEX root = ../distinguishing-writeup.tex

\subsection{ A $\tilde{\Omega}(\sqrt{n})$-sample lower bound for symmetric convex bodies (slabs)} \label{sec:symmetric-lb}

Given a unit vector $v \in \mathbb{S}^{n-1}$ and a positive value $r>0$, we say that the \emph{symmetric slab of width $2r$ in direction $v$} is the symmetric convex set $\Slab_{v,r} := \{x \in \R^n: |v \cdot x| \leq r\}.$  
\rnote{move to prelims?}

Our second lower bound shows that $\Omega(\sqrt{n}/\log n)$ samples are needed to distinguish $N(0,I_n)$ from $N(0,I_n)|_K$ where $K$ is an unknown symmetric slab that is promised to have volume roughly $1/2$:

\begin{theorem} \label{thm:lb-slab}
Let $A$ be any algorithm which is given access to samples from an unknown distribution ${\cal D}$ and has the following performance guarantee:

\begin{enumerate}

\item If ${\cal D}=N(0,I_n)$, then with probability at least $9/10$ the algorithm outputs ``un-truncated'';

\item If ${\cal D}=N(0,I_n)|_K$ where $K$ is an unknown symmetric slab with $\vol(K) \in [0.49,0.51]$, then with probability at least $9/10$ the algorithm outputs ``truncated.''

\end{enumerate}
Then $A$ must use at least $\Omega(\sqrt{n}/\log n)$ samples from ${\cal D}$.
\end{theorem}


\begin{proof}
Let $\psi: \R \to \{0,1\}$ be the function $\psi(t) = \Indicator[|t| \leq c]$ where $c \approx 0.68$ is the real number satisfying $\Pr_{\bg \sim N(0,1)}[|\bg| \leq c]=1/2.$
We define a distribution ${\cal K}$ over symmetric slabs as follows: to draw a symmetric slab $\bK \sim {\cal K}$, first draw a standard Normal vector $\bg \sim N(0,I_n)$, and let $\bK=\bK_{\bg}$ be the symmetric slab $\bK = \{x \in \R^n: \psi({\frac {\bg}{\sqrt{n}}} \cdot x)=1\}.$

We observe that given a particular outcome $g$ of $\bg$, the width of the slab $K=\bK_{g}$ is ${\frac {2c \sqrt{n}}{\|g\|}}$, and hence the volume $\vol(K)$ is $\Pr_{\bx \sim N(0,1)}[|\bx| < {\frac {c \sqrt{n}}{\|g\|}}].$ Standard tail bounds on the chi-distribution (which is the distribution of $\|\bg\|$ for $\bg \sim N(0,I_n)$) imply that $\Pr_{\bK \sim {\cal K}}[\vol(\bK) \notin [0.49,0.51]]$ is extremely small, in particular at most $1/n^{\omega(1)}$. 
Hence to prove \Cref{thm:lb-slab}, it suffices to prove an $\Omega(\sqrt{n} / \log n)$ lower bound on the sample complexity of any algorithm $A$ that outputs ``un-truncated'' with probability at least $9/10$ if it is given samples from $N(0,I_n)$ and outputs ``truncated'' with probability at least $91/100$ if it is given samples from $N(0,I_n)|_{\bK}$ where $\bK \sim {\cal K}$. We do this in the rest of the proof.

We consider two different distributions, ${\cal D}_1$ and ${\cal D}_2$, each of which is a distribution over sequences of $m=c\sqrt{n} / \log n$  points in $\R^n$:

\begin{enumerate}

\item A draw of $\overline{\bx}=(\bx^1,\dots,\bx^{m})$ from ${\cal D}_1$  is obtained by having each $\bx^i \in \R^n$ be distributed independently according to $N(0,I_n)$.

\item A draw of $\overline{\bx}=(\bx^1,\dots,\bx^{m})$ from ${\cal D}_2$ is obtained by drawing (once and for all) a set $\bK=\bK_{\bg} \sim {\cal K}$ (so $\bg \sim N(0,I_n)$) and having each $\bx^i$ be distributed independently according to $N(0,I_n)|_{\bK}$, i.e. each $\bx^i$ is drawn from $N(0,I_n)$ conditioned on  satisfying $\psi({\frac {\bg}{\sqrt{n}}} \cdot x)=1.$
\end{enumerate}

We further define two more distributions ${\cal D}'_1$ and ${\cal D}'_2$, each of which is a distribution over sequences of $3m$ points in $\R^n$:

\begin{enumerate}

\item A draw of $\overline{\bx}=(\bx^1,\dots,\bx^{3m})$ from ${\cal D}'_1$ is obtained as follows: $\bx^i$ is taken to be $\bb_i \bg^i$ where each $\bb_i$ is an independent uniform draw from $\zo$ and each $\bg^i$ is an independent draw from $N(0,I_n)$.

\item A draw of $\overline{\bz}=(\bz^1,\dots,\bz^{3m})$ from ${\cal D}'_2$ is obtained as follows:  once and for all draw $\bg \sim N(0,I_n)$, and take $\bz^i$ to be $\bg^i \cdot \psi({\frac {\bg}{\sqrt{n}}} \cdot \bg^i)$ where each $\bg^i$ is an independent draw from $N(0,I_n)$.

\end{enumerate}


Suppose that algorithm $A$ successfully distinguishes between ${\cal D}_1$ and ${\cal D}_2$, i.e. it outputs ``un-truncated'' with probability at least 9/10 when run on a draw from ${\cal D}_1$ and outputs ``truncated'' with probability at least 91/100 when run on a draw from ${\cal D}_2.$
We claim that then there is an algorithm $A'$ which successfully distinguishes between ${\cal D}'_1$ and ${\cal D}'_2$, i.e. it outputs ``un-truncated'' with probability at least 89/100 when run on a draw from ${\cal D}'_1$ (recall that this is a sequence of $3m$ points in $\R^n$) and outputs ``truncated'' with probability at least 90/100 when run on a draw from ${\cal D}'_2.$  This algorithm $A'$ simply takes the first $m$ nonzero points in its $3m$-point input sequence and uses them as input to $A$.  (We may suppose that $A'$ fails if there are fewer than $m$ nonzero points in the $3m$-point sample; it is easy to see that whether the input to $A'$ is drawn from ${\cal D}'_1$ or ${\cal D}'_2$, the probability of failure is at most $1/n^{\omega(1)}$ and hence is negligible.)  If the input sequence is a draw from ${\cal D}'_1$ then the input that $A'$ gives to $A$ is distributed according to ${\cal D}_1$, and if the input is a draw from ${\cal D}'_2$ then the input sequence that $A'$ gives to $A$ is distributed according to ${\cal D}_2$ (note that we may safely ignore the probability-0 event that some $\bg^i$ drawn from $N(0,I_n)$ is the zero vector).

Given the above claim, to prove \Cref{thm:lb-slab} it suffices to show that any algorithm $A'$ with the performance guarantee described above must have $3m = \Omega(\sqrt{n}/\log n).$  This follows from the statement
\begin{equation}
\label{eq:dtvprimes}
\text{If $m = c \sqrt{n}/\log n$, then~~~~}\dtv({\cal D}'_1,{\cal D}'_2) \leq 0.01.
\end{equation}
The rest of the proof establishes (\ref{eq:dtvprimes}).

Consider a coupling of the two distributions ${\cal D}'_1$ and ${\cal D}'_2$ as follows. A draw from the joint coupled distribution of $({\cal D}'_1,{\cal D}'_2)$ is generated in the following way:

\begin{itemize}

\item Let $(\bb_1,\dots,\bb_{3m})$ be a uniform random string from $\zo^{3m}$. 
\item Let $\bg, \bg^1,\dots,\bg^m$ be $3m+1$ independent draws from $N(0,I_n).$
\item The draw from the joint coupled distribution is $(\overline{\bx},\overline{\bz})$ where
\[
\text{for each $i =1,\dots,3m$,~~~}\bx^i = \bb_i \bg^i \quad \text{and}\quad
 \bz^i=\psi\left({\frac {\bg}{\sqrt{n}}} \cdot \bg^i\right) \bg^i .
\]
\end{itemize}
It is easily verified that this is indeed a valid coupling of ${\cal D}'_1$ and ${\cal D}'_2$.
We thus have
\begin{align}
\dtv({\cal D}'_1,{\cal D}'_2) 
&= \dtv((\bx^1,\dots,\bx^{3m}),(\bz^1,\dots,\bz^{3m})) \nonumber\\
&=\dtv\left((\bb_1\bg^1,\dots,\bb_{3m}\bg^{3m}),
\left(
\psi\left({\frac {\bg}{\sqrt{n}}} \cdot \bg^1\right) \bg^1,
\psi\left({\frac {\bg}{\sqrt{n}}} \cdot \bg^{3m}\right) \bg^{3m}
 \right)\right) \nonumber\\
 &\leq \dtv\left((\bb_1,\dots,\bb_{3m}),\left(\psi\left({\frac {\bg}{\sqrt{n}}} \cdot \bg^1\right),
 \dots, \psi\left({\frac {\bg}{\sqrt{n}}} \cdot \bg^{3m}\right)\right)\right) \label{eq:ham}
\end{align}
where the inequality uses the coupling described above. 
It remains to show that if $m = c \sqrt{n}/\log n$ then $(\ref{eq:ham}) \leq 0.01.$

We observe that for $\bg \sim N(0,I_n)$, we have that $\Pr[\psi(e_i \cdot \bg)=1]=\Pr[\psi(\bg_i)=1]=1/2$. Since the random variables $\{\bg_i\}_{i=1,\dots,3m}$ are independent, we have that the joint distribution of $(\bb_1,\dots,\bb_{3m})$ is identical to the joint distribution of $(\psi(e_1 \cdot \bg),\dots,\psi(e_{3m} \cdot \bg))$, namely, both distributions are uniform over $\zo^{3m}.$ Thus we have that
\begin{equation}
\label{eq:cheese}
(\ref{eq:ham}) = \dtv\left((\psi(e_1 \cdot \bg),\dots,\psi(e_{3m} \cdot \bg)),
\left(\psi\left({\frac {\bg^1}{\sqrt{n}}} \cdot \bg\right),
 \dots, \psi\left({\frac {\bg^{3m}}{\sqrt{n}}} \cdot \bg\right)\right)\right).
 \end{equation}
The rest of the argument proceeds similarly to the proof of \Cref{claim:dtvhalfspace} following (\ref{eq:humphrey}): briefly, for most outcomes $(g^1,\dots,g^{3m})$ of $\bg^1,\dots,\bg^{3m}$, the covariance structure of the two $3m$-dimensional Gaussians $(e_1 \cdot \bg,\dots,e_{3m} \cdot \bg)$ and $({\frac {g^1}{\sqrt{n}}} \cdot \bg,\dots,{\frac {g^{3m}}{\sqrt{n}}} \cdot \bg)$ are similar enough that we can bound the variation distance between those two Gaussians, which implies a bound on the variation distance between $(\psi(e_1 \cdot \bg),\dots,\psi(e_{3m} \cdot \bg))$ and $\left(\psi\left({\frac {g^1}{\sqrt{n}}} \cdot \bg\right),
 \dots, \psi\left({\frac {g^m}{\sqrt{n}}} \cdot \bg\right)\right)$. Details are given below.

We require a slight refinement of the notion of a ``good'' tuple of vectors from \Cref{sec:halfspace-lb} which now takes into account the lengths of the vectors as well as the angles between them. We say that a specific outcome $(g^1,\dots,g^{3m}) \in (\R^n)^{3m}$ of $(\bg^1,\dots,\bg^{3m}) \sim (N(0,I_n))^{3m}$ is \emph{atypical} if either

\begin{itemize}

\item [(a)] for some $i \in [3m]$ we have ${\frac {\|g^i\|}{\sqrt{n}}} \notin \left[1 - C_1 \sqrt{{\frac {\log n} n}},1 + C_1 \sqrt{{\frac {\log n} n}}\right],$ or

\item [(b)] for some pair $i\neq j$ we have $| {\frac {g^i \cdot g^j}{n}}| > C_1 \sqrt{{\frac {\log n} n}}$.

\end{itemize}
Otherwise we say that $(g^1,\dots,g^m)$ is \emph{typical}.  We defer the proof of the following claim until later:

\begin{claim} \label{claim:typical}
For a suitable choice of the absolute constant $C_1$, we have
$\Pr[(\bg^1,\dots,\bg^{3m})$ is atypical$]\leq 0.005.$
\end{claim}

Hence to show that $(\ref{eq:cheese}) \leq 0.01$ (and finish the proof of \Cref{thm:lb-slab} modulo \Cref{claim:typical}), it suffices to prove the following:

\begin{claim} 
\label{claim:pickwick}
Fix a typical $(g^1,\dots,g^{3m}) \in (\R^n)^{3m}$, where $m = c\sqrt{n}\log n$.
Then for $\bg \sim N(0,I_n)$ we have that
\begin{equation} \label{eq:persuasion}
\dtv\left((\psi(e_1 \cdot \bg),\dots,\psi(e_{3m} \cdot \bg)),
\left(\psi\left({\frac {g^1}{\sqrt{n}}} \cdot \bg\right),
 \dots, \psi\left({\frac {g^{3m}}{\sqrt{n}}} \cdot \bg\right)\right)\right) \leq 0.005.
\end{equation}
\end{claim}
Similar to \Cref{claim:hubert}, we prove \Cref{claim:pickwick} using \Cref{thm:DMR20}.
To apply \Cref{thm:DMR20} we take $\Sigma_1$ to be the identity matrix $I_{3m}$ and $\Sigma_2$ to be the $3m \times 3m$ matrix whose $(i,j)$ entry is ${\frac {g^i \cdot g^j}{n}}$, so a draw from $N(0,\Sigma_1)$ is distributed as $(e_1 \cdot \bg,\dots,e_{3m} \cdot \bg)$ and a draw from $N(0,\Sigma_2)$ is distributed as
$({\frac {g^1}{\sqrt{n}}} \cdot \bg,\dots, {\frac {g^{3m}}{\sqrt{n}}} \cdot \bg).$  Applying the data processing inequality for total variation distance, it follows that the LHS of (\ref{eq:persuasion}) is at most $\dtv(N(0^{3m},\Sigma_1),N(0^{3m},\Sigma_2))$.

Let $A$ denote the matrix $\Sigma_1^{-1}\Sigma_2 - I_{3m}$, so $\lambda_1^2,\dots,\lambda_{3m}^2$ are the eigenvalues of $A^2$  and we have $\sqrt{\lambda_1^2 + \cdots + \lambda_{3m}^2} = \sqrt{\tr(A^2))}.$
By part (a) of the definition of ``typical'' we know that each diagonal entry of $A$ has magnitude at most $3C_1 \sqrt{{\frac {\log n} n}}$, and by part (b) we know that each off-diagonal entry has magnitude at most $C_1 \sqrt{{\frac {\log n} n}}$.
The rest of the proof of \Cref{claim:pickwick} follows the proof of \Cref{claim:hubert} with obvious minor modifications.\rnote{Mutatis mutandis, one might say.}
\end{proof}

\medskip

\noindent \emph{Proof of \Cref{claim:typical}.} 
Recalling that $m=c\sqrt{n}/\log n$, a union bound together with \Cref{lem:johnstone} shows that for a suitable choice of $C_1$, part (a) of the ``atypical'' definition holds with probability at most 0.0025. 

For part (b), by a union bound over all ${m \choose 2}$ choices of $i \neq j$ and $m=c\sqrt{n}/\log n$, it is enough to show that for $\bg,\bg'$ independent $N(0,I_n)$ random variables we have
\begin{equation} \label{eq:goalproduct}
\Pr[\bg \cdot \bg' > C_1 \sqrt{n \log n}] < 1/n
\end{equation} (note that we have used the symmetry of the random variable $\bg \cdot \bg'$). By the radial symmetry of the $N(0,I_n)$ distribution we may assume that $\bg =(\br,0,\dots,0)$ where $\br^2 \sim \chi^2_n$, and hence (since $\bg'_1$ is distributed as $N(0,1)$) we have that $\bg \cdot \bg'$ is distributed as $\br \cdot N(0,1)$. By \Cref{lem:johnstone} we have that $\br^2 < 2n$ except with failure probability at most $\exp(-\Theta(n))$, so we may safely assume that $|r| \leq \sqrt{2}n.$ By the standard Gaussian tail bound $\Pr[N(0,1) \geq t] \leq e^{-t^2/2}$ for $t>0$, we see that \Cref{eq:goalproduct} holds for a suitable choice of the absolute constant $C_1$, and \Cref{claim:typical} is proved. \qed










==> sections/Anindya_s_folder/lower-bounds.tex <==
%!TEX root = distinguishing-writeup.tex
\newpage

\section{Glorious Lower Bounds}
\label{sec:prelims}


\input{lb-halfspaces}
\input{lb-slabs}
\input{lb-mixtures}


==> sections/Anindya_s_folder/prelims.tex <==
%!TEX root = distinguishing-writeup.tex



\section{Glorious Preliminaries}
\label{sec:prelims}

\subsection{Useful tools}

\rnote{Get rid of whatever of the following we don't need/use}

\paragraph{Notation.}
We use boldfaced letters such as $\bx, \boldf,\bA$, etc. to denote random variables (which may be real-valued, vector-valued, function-valued, set-valued, etc; the intended type will be clear from the context).
We write ``$\bx \sim \calD$'' to indicate that the random variable $\bx$ is distributed according to probability distribution $\calD.$ 

\paragraph{Geometry.}
For $r >0$, we write $S^{n-1}(r)$ to denote the origin-centered sphere of radius $r$ in $\R^n$ %adam420: changed this to parallel next line, the definition for the ball
and $\Ball(r)$ to denote the origin-centered ball of radius $r$ in $\R^n$, i.e.,
$$
S^{n-1}(r) = \big\{x \in \R^n: \|x\|=r\big\}\quad\text{and}\quad
 %Define ball $B^n(r)$. Maybe skip the superscript $n-1$ and $n$.
%We write
% i.e.
\Ball(r) = \big\{x \in \R^n : \|x\| \leq r\big\},
$$
%When $r=1$ we simply write $\Ball$ for $\Ball(1).$  We similarly write $\Sphere(r)$ to denote $\{(x_1,\dots,x_n) \in \R^n: \sum x_i^2 = r^2\}$ and $\Sphere$ for $\Sphere(1).$
where $\|x\|$   denotes the $\ell_2$-norm $\|\cdot \|_2$ of $x\in \R^n$.
We also write $S^{n-1}$ for the unit sphere $S^{n-1}(1)$. % for convenience.


Recall that a set $C \subseteq \R^n$ is convex if $x,y \in C$ implies $\alpha\hspace{0.03cm}x + (1-\alpha) y \in C$ for all $\alpha\in [0,1].$ 
%We write $\calC_\convex$ to denote the class of all convex sets in $\R^n.$
Recall that convex sets are Lebesgue measurable.
%Given a set $C \subseteq \R^n$ we write $\Conv(C)$ to denote the convex hull of $C$.


For sets $A,B \subseteq \R^n$, we write $A + B$ to denote the Minkowski sum $\{a + b: a \in A\ \text{and}\ b \in B\}.$ For a set $A \subseteq \R^n$ and $r > 0$ we write $rA$ to denote the set $\{ra : a \in A\}$.
Given a point $a$ and a set $B\subseteq \R^n$, we use $a+B$ and $B-a$ to denote
  $\{a\}+B$ and $B+\{-a\}$ for convenience.  
\ignore{
%For a convex set $C$, 
%  %(i.e. a convex set such that $\sup_{c \in C} \|c\| \leq K$ for some real value $K$), 
%  we write $\partial C$ to denote its \emph{boundary}, i.e. the set of points $x \in \R^n$ such that for all $\delta > 0$,
%  the set $x + \Ball(\delta)$ contains at least one point in $C$ and at least one point outside $C$.\ignore{\red{For a bounded convex set $C$ (i.e. a convex set such that $\sup_{c \in C} \|c\| \leq K$ for some real value $K$), we write $\partial C$ to denote its \emph{boundary}, i.e., \blue{the set of points $x\in C$ such that
%  $x+\Ball(\delta)\not\subseteq C$ for any $\delta>0$}.\xnote{Added a definition of the boundary. Hope this
%  is the one we use here.}}\rnote{Maybe we should write \blue{the set of points $x \in \R^n$ such that for all $\delta > 0$,
%  the set $x + \Ball(\delta)$ contains at least one point in $C$ and at least one point outside $C$}.  Otherwise I think with the current definition if $C$ is (say) an open ball $\{x: \|x\| < r\}$  there would be no points satisfying the definition of the boundary.}}
%\vspace{-0.2cm}
}

\paragraph{Probability.}
%We use $\normal^n$ to denote the standard $n$-dimensional Gaussian distribution with zero mean and identity covariance matrix. We also recall that the probability density function for the one-dimensional Gaussian distribution is $$\varphi(x) = {\frac 1 {\sqrt{2 \pi}}}\cdot \exp(-x^2/2).$$
%Sometimes we denote $\normal^n$ by $\gaus$ for convenience.
We write $\vol(K)$ to denote the Gaussian volume of a \rnote{Borel/Lebesgue measurable?} set $K \subseteq \R^n$, i.e. $\vol(K) = \Pr_{\bx \sim N(0,I_n)}[\bx \in K].$  For a \rnote{Borel/Lebesgue measurable?}  set $K \subseteq \R^n$, we write $N(0,I_n)|_K$ to denote the standard Normal distribution conditioned on $K$, so the pdf of $N(0,I_n)|_K$ is $\varphi_n(x)/\vol(K)$ where $\varphi_n(x) = (2\pi)^{-n/2} e^{-\|x\|^2/2}$ is the standard Gaussian pdf.

The squared norm $\|\bx\|^2$ of $\bx \sim N(0,I_n)$ is distributed according to the chi-squared distribution $\chi_n^2$
  with $n$ degrees of freedom.  The following tail bound for $\chi_n^2$ (see \cite{Johnstone01}) will be useful:

\begin{lemma} [Tail bound for the chi-squared distribution] \label{lem:johnstone}
Let $\bX \leftarrow \chi_n^2$. % be a chi-squared random variable with $n$ degrees of freedom. Then
Then we have
$$\Pr\big[|\bX-n| \geq tn\big] \leq e^{-(3/16)nt^2},\quad\text{for all $t \in [0, 1/2)$.}$$
\end{lemma}




\subsection{Convex influences}
Define convex influence

\medskip

State our Poincare:

\begin{proposition}
	For CSC $K\subseteq\R^n$ with $\rinn > 0$ (and hence $\Var[K] > 0$), we have 
	\rnote{We could just give the $		\TInf[K] \geq \Omega\pbra{\rinn\cdot\Var[K]}$ version here if we prefer}
	
	\begin{equation} \label{eq:kkl}
		\TInf[K] \geq \Omega\pbra{\rinn\cdot\Var[K]\sqrt{\log\pbra{\frac{1}{\Var[K]}}}}.
	\end{equation}
\end{proposition}

\subsection{The classes of distributions we consider}

A set $K \subseteq \R^n$ is \emph{symmetric} if for all $x$ we have $x \in K$ if and only if $-x \in K$. Similarly, we say that a distribution over $\R^n$ with pdf $\phi$ is symmetric if $\phi(x)=\phi(-x)$ for all $x$.

We let $\Psymm$ denote the class of all distributions $N(0,I_n)|_K$ where $K \subseteq \R^n$ may be any symmetric convex set, $\Pconv$ denote the class of all such distributions where $K$ may be any convex set (not necessarily symmetric), and $\Pltf$ denote the class of all such distributions where $K$ may be any \rnote{origin-centered? or general? Should get the positive result for general LTFs if we can} linear threshold function $\sign(v \cdot x \geq \red{\theta}).$ We let $\Mix$ denote the class of all convex combinations of distributions from $\Psymm$, and we remark that a distribution in $\Mix$ can be viewed as $N(0,I_n)$ conditioned on a \emph{mixture} of symmetric convex sets.

The following alternate characterization of $\Mix$ may be of interest.  Let $\Plcg$ denote the class of all symmetric distributions that are log-concave relative to the standard Normal distribution, i.e. all distributions that have a pdf of the form $e^{-\tau(x)} \varphi_n(x)$ where $\tau(\cdot)$ is a symmetric convex function. Let $\Mixlcg$ denote the class of all mixtures of distributions in $\Plcg.$

\begin{claim} 
$\Mixlcg=\Mix.$
\end{claim}
\begin{proof}
We will argue below that $\Plcg \subseteq \Mix.$ Given this, it follows that any mixture of distributions in $\Plcg$ is a mixture of distributions in $\Mix$, but since a mixture of distributions in $\Mix$ is itself a distribution in $\Mix$, this means that $\Mixlcg \subseteq \Mix.$ For the other direction, we observe that any distribution in $\Psymm$ belongs to $\Plcg$ (recall that a distribution in $\Psymm$ has a pdf which is $\Indicator[x \in K] \varphi_n(x)$ for some symmetric convex $K$) and hence $\Mix \subseteq \Mixlcg.$

Fix any distribution ${\cal D}$ in $\Plcg$ and let $e^{-\tau(x)}\varphi_n(x)$ be its pdf. We have that
\begin{equation} \label{eq:lolly}
e^{-\tau(x)} \varphi_n(x) = \E[A_{\bt}(x)] \cdot \varphi_n(x)
\end{equation}
where $A_t(x) = \Indicator[e^{-\tau(x)} \geq t]$ and the expectation in (\ref{eq:lolly}) is over a uniform $\bt \sim [0,1]$. Since $\tau$ is a symmetric convex function we have that the level set $\{x \in \R^n: e^{-\tau(x)} \geq t\}$ is a symmetric convex set, so ${\cal D}$ is a mixture of distributions in $\Psymm$ as claimed above.
\end{proof}





==> sections/curvy.tex <==
%!TEX root = ../distinguishing-writeup.tex



\begin{figure}
\centering 

\begin{tikzpicture}
	\def\lambdaPlot{\x,{(2.71^(-\x/3))*(\x-1)*\x^(1/2)}}
	\def\chiPlot{\x,{4+(2.71^(-\x/2))*(1/8)*\x^(3)}}
	
	% BOTTOM 
	\fill[fill=blue!5] (1.75,0) -- plot[domain=1.75:13] (\lambdaPlot) -- (13,0) -- cycle;
	\node (area) at (6, 0.75){Area $= 1$};
	\fill[pattern=north west lines,pattern color=black!25] (0,0) -- plot[scale=1,domain=0:1,smooth,] (\lambdaPlot) -- (1,0);
	\fill[pattern=north east lines,pattern color=black!25] (0,0) -- plot[scale=1,domain=1:1.75,smooth,] (\lambdaPlot) -- (1.75,0);
	\draw[->] (0,0) -- (14, 0) node[right] {$R$};
	\filldraw[black] (0,0) circle (1pt) node[anchor=east]{$0$};
	\filldraw[black] (1,0) circle (1pt) node[anchor=north]{$\frac{1}{\delta}$};
	\filldraw[black] (1.75,0) circle (1pt) node[anchor=north west]{$a^\ast$};
%	\draw[scale=1, domain=0:13, smooth, variable=\x, black] plot (\lambdaPlot);
	\draw [dashed] plot[scale=1,domain=0:1.75,smooth] (\lambdaPlot);
	\draw [] plot[scale=1,domain=1.75:13,smooth] (\lambdaPlot);
	\node (lambda) at (13, 1){$\lambda(R)$};

	% TOP
	\fill[fill=pink!75] (0,4) -- plot[domain=0:1.75] (\chiPlot) -- (1.75,4) -- cycle;
	\draw[->] (0,4) -- (14, 4) node[right] {$x$};
	\filldraw[black] (0,4) circle (1pt) node[anchor=east]{$0$};
	\filldraw[black] (1.75,4) circle (1pt) node[anchor=north west]{$a^\ast$};
	\draw plot[scale=1,domain=0:13,smooth] (\chiPlot);
	\node (S) at (13, 5){$S(x) = p(x)$ for $x\geq a^\ast$};
	
	% ACROSS
	\draw[dotted] (1.75,4.279) -- (1.75,0.56);
	\draw[] (1.75,0) -- (1.75,0.555);
	
	% LABEL
	\filldraw [color=black,fill=pink!75] (4,6) rectangle ++(0.75,0.5);
	\node (label) at (1.5,6.25) {$\dtv\pbra{S,\chi^2(n, (1+\delta')^{-1}} \leq $};
\end{tikzpicture}

\caption{Constructing the mixture distribution $S$. The bottom plot, of $\lambda(R)$, is the function defined by \Cref{eq:first-lambda-formula}; $a^\ast$ is the value for which the two cross-hatched areas are the same.  The revised definition of $\lambda(R)$ given in \Cref{def:lambdaR}, together with \Cref{eq:eggs}, determines $S$, depicted in the top plot.
}
\label{fig:lambda}
	
\end{figure}

%\begin{tikzpicture}[scale = 0.925]
%\filldraw[rotate around={45:(0,0)}, fill=pink!20!blue!20] (-1.25,0) ellipse (2.5 and 1.5);
%\path[pattern=north west lines,pattern color=black!25] (2,3) -- (2.75,3) -- (2.75,-3) -- (2,-3);
%\draw[->] (-4,0)--(3,0) node[above]{$e_1$};
%\draw[->] (0,-3)--(0,3) node[above]{$e_2$};
%\draw[-] (2,-3)--(2,3);	
%\filldraw[black] (0,0) circle (1pt) node[anchor=north east]{$(0,0)$};
%\filldraw[black] (2,0) circle (1pt) node[anchor=north west]{$(0.1,0)$};
%\filldraw[black] (-1.1,-1.1) circle (1pt) node[anchor=north]{$(\mu_1,\mu_2)$};
%\node at (-3.25,-2) {$K$};
%\node at (0,-4) {(a)};
%
%\end{tikzpicture}

==> sections/halfspaces.tex <==
%!TEX root = ../distinguishing-writeup.tex

\section{An 
$O(\sqrt{n}/\eps^2 + (\log(1/\eps))^2/\eps^4)$-Sample Algorithm for LTFs}
\label{sec:halfspaces}

In this section, we obtain a distinguisher for LTFs with better sample complexity than the distinguisher for convex sets ($(O(\sqrt{n})$ versus $O(n)$). More precisely, we have the following: 

\begin{theorem} \label{thm:LTF}
There is an algorithm \LTF\ (\Cref{alg:halfspaces}) with the following performance guarantee:  Given any $\eps > 0$ and access to independent samples from any unknown distribution ${\cal D} \in \Pltf$, the algorithm uses $O(\sqrt{n}/\eps^2 + (\log(1/\eps))^2/\eps^4)$ samples, and

\begin{enumerate}

\item If ${\cal D}=N(0,I_n)$, then with probability at least $9/10$ the algorithm outputs ``un-truncated'';

\item If $\dtv\pbra{{\cal D}, N(0,I_n)} \geq \eps$, then with probability at least $9/10$ the algorithm outputs ``truncated.''

\end{enumerate}

\end{theorem}

Looking ahead, we will show in \Cref{thm:lb-ltf} that this is essentially the best possible sample complexity. The intuition behind \LTF~starts with the easy observation that the center of mass of a LTF-truncated Gaussian is not at the origin. Employing \Cref{prop:mean-estimator} to estimate the center of mass, however, results in a $O(n)$-sample complexity, matching that of \Cref{alg:convex}. We therefore employ a different statistic, namely the \emph{norm} of the empirical center of mass (cf. \Cref{eq:intro-ltf-statistic}), which allows us to successfully distinguish LTF-truncated Gaussians using fewer samples.

\begin{algorithm}[t]
\caption{Distinguisher for LTFs}
\label{alg:halfspaces}
\vspace{0.5em}
\textbf{Input:} $\calD\in\Pltf$, $\eps > 0$\\[0.5em]
\textbf{Output:} ``Un-truncated'' or  ``truncated''

\ 

\LTF$(\calD, \epsilon)$:
\begin{enumerate}
    \item Let $T := {\frac {C \sqrt{n}}{ \eps^2}} + {\frac {C (\log(1/\eps))^2}{\eps^4}} $ and sample $\x{1},\ldots,\x{T} \sim \calD$.
    \item Set $\bN := \vabs{\frac{1}{T}\sum_{i=1}^T \x{i}}^2$.
    \item Output ``truncated'' if $\bN\geq {\frac n T} + c \eps^2$, and ``un-truncated'' otherwise.
\end{enumerate}

\end{algorithm}



\subsection{Moments of Univariate Truncated Gaussians}

Our proof of \Cref{thm:LTF} will rely on expressions for the first four moments of the truncated univariate standard Gaussian distribution. We start by introducing some convenient notation. 

\begin{definition}
	For $b\in\R$, the \emph{Mills ratio} $\Mills{b}$ is
	\[\Mills{b} := \frac{1-\Phi(b)}{\phi(b)}.\]
\end{definition}

\begin{notation}
	Let $K := [b, \infty) \sse\R$, and let $\bx \sim N(0, 1)|_K$. We write $\calM_b(p)$ for the $p^\text{th}$ raw moment of $\bx$, i.e. 
	\[\calM_p(b) := \Ex_{\bx \sim N(0, 1)|_K}\sbra{\bx^p}.\]
	When $b$ is clear from context, we will simply write $\calM_p$ instead. 
\end{notation}

 The following expressions can be obtained via repeated integration by parts; alternatively, see \cite{Orjebin2014}.

\begin{fact}[Moments of truncated Gaussian]
\label{fact:truncated-gaussian-moments}
	Let $K := [b, \infty) \sse\R$, and let $\bx \sim N(0, 1)|_K$. Then
	\[
	\calM_1 = \frac{1}{\Mills{b}},\quad
	\calM_2 = 1 + \frac{b}{\Mills{b}},\quad
	\calM_3 = \frac{2+b^2}{\Mills{b}},\quad\text{and}\quad
	\calM_4 = 3 + \frac{b^3 + 3b}{\Mills{b}}.
	\]
\end{fact}

%%%%%%%%%%%%%%%% SLICK THING %%%%%%%%%%%%%%%%%%%%%
%The following lemma is a straightforward calculation whose proof we omit.\snote{See \url{https://visit.randy.city/post/2020/variance-of-sample-mean-squared}.}
%
%\begin{lemma} \label{lemma:variance-LTF-formula}
%	Let $\calD$ be an arbitrary univariate distribution. Then we have 
%	\[\Varx_{\x{j}\sim\calD}\sbra{\pbra{\frac{1}{m}\sum_{j=1}^T \x{j}}^2} = \frac{4\mu}{m}\sigma^2 + \frac{4\mu}{T^2}\Ex\sbra{(\bx-\mu)^3} + \pbra{\frac{2m-3}{T^3}}\sigma^4 + \frac{1}{T^3}\Ex\sbra{(\bx-\mu)^4},\]
%	where $\mu := \Ex\sbra{\bx}$ and $\sigma^2 := \Varx\sbra{\bx}$ for $\bx\sim\calD$.
%\end{lemma}

Standard tail bounds on the Gaussian distribution (see e.g. \cite{wainwright_2019}) imply that
\begin{equation} \label{eq:lower-bound-on-mills}
	\frac{1}{x} \geq \Mills{x} \geq \frac{x}{1+x^2} \qquad\text{for } x\geq 0.
\end{equation}
It is also easy to check that 
\begin{equation} \label{eq:neg-mills}
	\Mills{x} \geq \sqrt{\frac{\pi}{2}} \qquad\text{for } x< 0.
\end{equation}

We will also require the following estimate on the \emph{Gaussian isoperimetric function} $\phi\circ\Phi^{-1}(\cdot)$, a proof of which can be found in Proposition~27 of \cite{DNS21influence22}.

\begin{proposition} \label{prop:GIP-bound}
	For all $\eps\in(0,1)$, we have 
	\[\phi\circ{\Phi^{-1}(\eps)}\geq\sqrt{\frac{2}{\pi}}\min\cbra{\eps,1-\eps}.\]
\end{proposition}


\subsection{Proof of \Cref{thm:LTF}}

We can now proceed to the proof of \Cref{thm:LTF}.

\begin{proof}[Proof of \Cref{thm:LTF}]
Suppose first that $\calD=N(0,I_n)$. Writing $\overline{\bx}$ for the empirical mean $\frac{1}{T}\sum_{i=1}^T \x{i}$, it is clear that $\E[\overline{\bx}]=0^n$ (the expected location of the empirical mean vector is the origin). Let $\bN$ be the random variable which is the square of the Euclidean distance from $\overline{\bx}$ to the origin, i.e. $\bN=\|\overline{\bx}\|^2.$ Then 
\begin{equation}\label{eq:mean-ltf-untrunc}
\E[\bN]=
\E\left[\sum_{i \in [n]} \overline{\bx}_i^2\right]=
\E\left[ \sum_i \left(\sum_{j=1}^T {\frac {\x{j}_i}{T}}\right)^2\right]
= \E\left[{\frac 1 {T^2}}\sum_i \sum_{j_1,j_2} \x{j_1}_i \x{j_2}_i  \right]=\frac{n}{T},
\end{equation}
and the variance of $\bN$ is
\[
	\Var[\bN] = \Var\left[\sum_{i=1}^n \overline{\bx}_i^2\right]=n\cdot\Var\left[\overline{\bx}_1^2\right] 
	= n\cdot\left(\E\left[\overline{\bx}_1^4\right]-\E\left[\overline{\bx}_1^2\right]^2\right).
\]
%%%%%%%%%% SLICK BUT USELESS THING? %%%%%%%%%%%%%%%%
%Applying \Cref{lemma:variance-LTF-formula} with $\mu = 0$ and $\sigma^2 = 1$, we get that 
%\[\Var\sbra{\overline{x}_1^2} = \frac{1}{T^3}\pbra{(2m-3) + \Ex_{\bx\sim N(0,1)}\sbra{\bx^4}} = \frac{2}{T^2}.\]
%It follows that 
%\begin{equation} \label{eq:var-ltf-untrunc}
%\Var[\bN] = n\left(\frac{3}{T^2} - \frac{1}{T^2}\right) = \frac{2n}{T^2}.
%\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Note that $\E\left[\overline{\bx}_1^2\right] = \frac{1}{T}$, and that 
\[
	\E\left[\overline{\bx}_1^4\right] = \E\left[\left(\frac{1}{T}\sum_{j=1}^T \x{j}_1\right)^4\right]\\
	=\frac{1}{T^4} \sum_{i,j,k,l=1}^T \E\left[\x{i}_1 \x{j}_1\x{k}_1\x{l}_1\right].
\]
Note that we have a non-zero contribution to the sum in the final expression above when
\begin{itemize}
	\item $i=j=k=l$ with $\E\left[\x{i}_1 \x{j}_1\x{k}_1\x{l}_1\right] = 3$, contributing $3T$ to the sum; and 
	\item $i$ equals exactly one of the other three indices (there are three ways to choose which one) and the other two are equal; in this case $\E\left[\x{i}_1 \x{j}_1\x{k}_1\x{l}_1\right] = 1$, so these contribute $3(T^2-T)$ to the sum.
\end{itemize}
It follows that 
\begin{equation} \label{eq:var-ltf-untrunc}
\Var[\bN] = n\left(\frac{3}{T^2} - \frac{1}{T^2}\right) = \frac{2n}{T^2}.
\end{equation}


Now, suppose that ${\cal D} \in \Pltf$ with $\dtv(\calD, N(0,I_n))\geq\epsilon$. Thanks to spherical symmetry of the Gaussian distribution, we can assume that the halfspace is given by 
\[K := \{x\in\R^n : x_1 \geq b\}, \]
with $\Phi(b) \geq \eps$. 
%In particular, we have $b \leq \red{TODO}$ by \Cref{fact:1d-truncation-tail-bounds}. 
For this distribution, we have that 
\[\E[\overline{\bx}]=(\E[\bx_1],0,\dots,0)
\qquad\text{where}\qquad \bx_1 \sim N(0,1)_{[b,\infty)}.\]
As above let $\bN = \|\overline{\bx}\|^2$, and now we have that
\begin{align}
	\E[\bN]&=\E\left[\sum_{i \in [n]} \overline{\bx}_i^2\right] \nonumber\\
	&=\E\left[ \left(\sum_{j\in[T]} {\frac {\x{j}_1}{T}}\right)^2 \right] + 
\E\left[ \sum_{i=2}^n \left(\sum_{j \in [T]} {\frac {\x{j}_i}{T}}\right)^2\right] \nonumber\\
&={\frac 1 {T^2}} \sum_{j_1,j_2=1}^T\E\left[\x{j_1}_1 \x{j_2}_1\right] + \frac{(n-1)}{T} \nonumber\\
&=\pbra{\frac{\calM_2(b)}{T} + \frac{(T-1)\calM_1(b)^2}{T}} + \frac{(n-1)}{T} \label{eq:potato-chips}\\
&=\frac{n}{T} + \calM_1(b)^2 + \frac{\calM_1(b)}{T}\pbra{b - \calM_1(b)},\label{eq:haldiram}
\end{align}
where we used the expression for $\calM_2(b)$ from \Cref{fact:truncated-gaussian-moments}. When $\eps \geq 0.5$, we have $b\geq 0$ and that 
\[\Ex\sbra{\bN} \geq \frac{n}{T} + \Omega\pbra{1} = \frac{n}{T} + \Omega\pbra{\eps^2}\]
using \Cref{eq:lower-bound-on-mills}. On the other hand, when $\eps < 0.5$, we have $b< 0$; in this case, we have from \Cref{fact:truncated-gaussian-moments} and \Cref{prop:GIP-bound} that 
\[\calM_1(b) \geq \frac{\phi\circ\Phi^{-1}(\eps)}{1-\eps} = \Omega(\eps).\]
(Note that we used the fact that $\phi(x)$ is monotone increasing for $x\leq 0$.) 
Combining this with \Cref{eq:neg-mills} we also get that 
\[\frac{\calM_1(b)}{T}\pbra{b - \calM_1(b)} \geq \frac{\Omega(\eps)}{T}\pbra{b-\sqrt{\frac{2}{\pi}}}.\]
Recalling that since $\eps < 0.5$ we have $\Theta(\sqrt{\ln(1/\eps)})<b<0$, it follows from \Cref{eq:haldiram} and our choice of $T = C n / \eps^2$ that
\begin{equation}\Ex\sbra{\bN} \geq \frac{n}{T} + \Omega\pbra{\eps^2}. \label{eq:mean-ltf-trunc}
\end{equation}

Turning to the variance of $\bN$, we have 
\begin{equation} \label{eq:var-ltf-1}
	\Var\left[\sum_{i\in[n]}\overline{\bx}_i^2\right]=\Var\left[\overline{\bx}_1^2\right] + \sum_{i=2}^n\Var\left[\overline{\bx}_i^2\right] = \Var\left[\left(\sum_{j\in[T]}\frac{\x{j}_1}{T}\right)^2\right] + \frac{2(n-1)}{T^2}.
\end{equation}
Writing
\begin{align}
	\Var\left[\left(\sum_{j\in[T]}\frac{\x{j}_1}{T}\right)^2\right] &= \E\left[\left(\sum_{j\in[T]}\frac{\x{j}_1}{T}\right)^4\right] - \E\left[\left(\sum_{j\in[T]}\frac{\x{j}_1}{T}\right)^2\right]^2 \label{eq:zebra},
\end{align}
the contributions to the sum in the first term above, $\frac{1}{T^4}\sum_{i,j,k,\ell=1}^T\E\left[\x{i}_1\x{j}_1\x{k}_1\x{\ell}_1\right]$, break down as follows:
\begin{itemize}
	\item When $i=j=k=\ell$ the expectation is $\calM_4$; there are $T$ ways for this to happen so this contributes $T\calM_4$ to the sum;
	\item When three of the indices are equal and the fourth is distinct the expectation is $\calM_3\calM_1$; there are $4T(T-1)$ ways for this to happen so it contributes $4T(T-1)\calM_3\calM_1$ to the sum;
	\item When two indices equal each other and so do the other two the expectation is $\calM_2^2$; there are $3T(T-1)$ ways for this to happen so it contributes $3T(T-1)\calM_2^2$ to the sum;
	\item When two indices equal each other and the other two are two distinct values, the expectation is $\calM_2\calM_1^2$; there are $6T(T-1)(T-2)$ ways for this to happen so it contributes $6T(T-1)(T-2)\calM_2\calM_1^2$ to the sum;
	\item When all four indices are distinct the expectation is $\calM_1^4$; there are $T(T-1)(T-2)(T-3)$ ways for this to happen so it contributes $T(T-1)(T-2)(T-3)\calM_1^4$ to the sum.
\end{itemize}
In particular, we have 
\begin{equation}
	\label{eq:variance-first-term}
	\E\left[\left(\sum_{j\in[T]}\frac{\x{j}_1}{T}\right)^4\right] \leq O\pbra{\frac{\calM_4}{T^3} + \frac{\calM_3\calM_1 + \calM_2^2}{T^2} +\frac{\calM_2\calM_1^2}{T}} + \calM_1^4.
\end{equation}
We also have from \Cref{eq:potato-chips} and \Cref{fact:truncated-gaussian-moments} that 
\begin{align}
\E\left[\left(\sum_{j\in[T]}\frac{\x{j}_1}{T}\right)^2\right]^2 &= \pbra{\frac{\calM_2}{T} + \frac{(T-1)\calM_1^2}{T}}^2	\nonumber \\
&= \pbra{\calM_1^2  + \frac{(\calM_2-\calM_1^2)}{T}}^2. \label{eq:variance-second-term}
\end{align}
It follows from \Cref{eq:zebra,eq:variance-first-term,eq:variance-second-term} that 
\begin{equation} \label{eq:variance-ltf-last}
	\Var\left[\left(\sum_{j\in[T]}\frac{\x{j}_1}{T}\right)^2\right] \leq O\pbra{\frac{\calM_4}{T^3} + \frac{\calM_3\calM_1 + \calM_2^2}{T^2} +\frac{\calM_2\calM_1^2 + \calM_1^4}{T}}.
\end{equation}
Recalling \Cref{eq:var-ltf-1}, when $\eps \geq 0.5$ (i.e. $b\geq 0$) we have that the RHS of \Cref{eq:variance-ltf-last} is 
\begin{equation}
\label{eq:poutine}\eqref{eq:variance-ltf-last} \leq O\pbra{\frac{\calM_1^4}{T}} = O\pbra{\frac{b^4}{T}}\quad\text{and so}\quad \Var\left[\sum_{i\in[n]}\overline{\bx}_i^2\right] \leq O\pbra{\frac{n}{T^2} + \frac{b^4}{T}} \leq
O\pbra{\frac{n}{T^2} + \frac{\log(1/\eps)^2}{T}},
\end{equation}
where we used $|b| \leq \Theta(\sqrt{\log(1/\eps)})$ for the last inequality.
On the other hand, when $\eps < 0.5$ (i.e. $b< 0$) we have that the RHS of \Cref{eq:variance-ltf-last} is 
\[O\pbra{\frac{1}{T} + \frac{1}{T^2}} \qquad\text{and so}
\qquad
\Var\left[\sum_{i\in[n]}\overline{\bx}_i^2\right] \leq O\pbra{\frac{n}{T^2} + \frac{1}{T}}.\] 

Summarizing \Cref{eq:mean-ltf-untrunc}, \Cref{eq:var-ltf-untrunc}, \Cref{eq:mean-ltf-trunc} and \Cref{eq:poutine}, we have that

\begin{align*}
	\mathbf{E}[\bN ] &= {\frac n T} \quad\text{and}\quad &\Var[\bN] = \frac{2n}{T^2}& \qquad \text{when } \calD = N(0,I_n),\\
	\mathbf{E}[\bN ] &\geq {\frac n T} +\Omega(\epsilon^2) \quad\text{and}\quad &\Var[\bN] \leq O\pbra{\frac{n}{T^2} + \frac{\log(1/\eps)^2}{T}}& \qquad \text{when } \dtv(\calD, N(0,I_n))\geq\epsilon.
\end{align*}
 
The correctness of \Cref{alg:halfspaces} follows by our choice of $T = C\sqrt{n}/\epsilon^2$ (for a sufficiently large constant $C$) and Chebyshev's inequality.  This finishes the proof. 
%\bigskip \bigskip \bigskip
%
%\red{Therefore taking $T = O\max\cbra{\frac{\sqrt{n}}{\eps^2}, \log^2\pbra{\frac{1}{\eps}}}$ allows us to distinguish between $\calD_G$ and $\calD_T$ via Chebyshev's inequality.} 
\end{proof}






==> sections/lb-halfspaces-garbage.tex <==
%!TEX root = ../distinguishing-writeup.tex

\subsection{A $\tilde{\Omega}(\sqrt{n})$-Sample Lower Bound for Halfspaces} \label{sec:halfspace-lb}

Our first lower bound, \Cref{thm:lb-ltf}, shows that $\Omega(\sqrt{n}/\log n)$ samples are needed to distinguish $N(0,I_n)$ from $N(0,I_n)|_K$ where $K$ is an unknown halfspace whose separating hyperplane passes through the origin. 
Some of the ideas in this lower bound will recur in our lower bound for symmetric ``slabs'' (intersections of two parallel halfspaces) given in \Cref{sec:symmetric-lb}, but by taking advantage of the fact that origin-centered halfspaces are odd functions, we can sidestep some aspects of the argument that arise for slabs; hence we give a self-contained proof for halfspaces below.

\begin{theorem} \label{thm:lb-ltf}
Let $A$ be any algorithm which is given access to samples from an unknown distribution ${\cal D}$ over $\R^n$ and has the following performance guarantee:

\begin{enumerate}

\item If ${\cal D}=N(0,I_n)$, then with probability at least $2/3$ the algorithm outputs ``un-truncated'';

\item If ${\cal D}=N(0,I_n)|_K$ where $K$ is an unknown zero-threshold LTF, then with probability at least $2/3$ the algorithm outputs ``truncated.''

\end{enumerate}
Then $A$ must use at least $\Omega(\sqrt{n}/\log n)$ samples from ${\cal D}$.
\end{theorem}

\begin{proof}
We consider two different distributions, ${\cal D}_1$ and ${\cal D}_2$, each of which is a distribution over sequences of $m$  points in $\R^n$.

\begin{enumerate}

\item A draw of $\overline{\bx}=(\bx^1,\dots,\bx^m)$ from ${\cal D}_1$  is obtained by having each $\bx^i \in \R^n$ be distributed independently according to $N(0,I_n)$.

\item A draw from ${\cal D}_2$ is obtained by independently drawing $\bg,\bg^1,\dots,\bg^m$ from  $N(0,I_n)$ and outputting $(\sign(\bg \cdot \bg^1) \bg^1, \dots, \sign(\bg\cdot \bg^m) \bg^m).$
\end{enumerate}

Observe that a draw from ${\cal D}_2$ is distributed as a sample of $m$  independent draws from $N(0,I_n)|_{\bK}$ where $\bK=\{x \in \R^n: \bg \cdot x \geq 0\}$ is a random zero-threshold LTF defined by a normal vector $\bg$ that is drawn from $N(0,I_n)$ (here is where we are using that any zero-threshold LTF is an odd function). Thus to prove \Cref{thm:lb-ltf} it suffices to show that any algorithm that determines  (with correctness probability at least $2/3$) whether an $m$-element sample came from ${\cal D}_1$ or ${\cal D}_2$ must have $m = \Omega(\sqrt{n}/\log n).$ This is an immediate consequence of the following claim: 

\begin{claim}
\label{claim:dtvhalfspace}
There is a universal constant $c>0$ such that for $m = c \sqrt{n}/\log n$, we have 
$\dtv({\cal D}_1,{\cal D}_2) \leq 0.1.$
\end{claim}

\medskip
\noindent \emph{Proof of \Cref{claim:dtvhalfspace}.}
We first observe that a draw $(\bx^1,\dots,\bx^m) \sim {\cal D}_1$ is distributed identically to $(\bu_1 \bx^1,\dots,
\bu_m \bx^m)$ where each $\bu_i$ is an independent uniform $\bits$ random variable. Next, we observe that
\begin{align} 
\dtv({\cal D}_1,{\cal D}_2) &=
\dtv((\bu_1 \bx^1,\dots,
\bu_m \bx^m),(\sign(\bg \cdot \bg^1) \bg^1, \dots, \sign(\bg\cdot \bg^m) \bg^m))\nonumber \\
&\leq\dtv((\bu_1,\dots,\bu_m),(\sign(\bg \cdot \bg^1),\dots,\sign(\bg \cdot \bg^m))) 
\tag{coupling $\overline{\bx}$ and $\overline{\bg}=(\bg^1,\dots,\bg^m)$} \nonumber
\end{align}
where $\bu=(\bu_1,\dots,\bu_m)$ is uniform over $\bits^m$. So it remains to bound the variation distance between the two $m$-bit strings $\bu$ and $(\sign(\bg \cdot \bg^1),\dots,\sign(\bg \cdot \bg^m)).$ We may view a uniform $\bu \sim \bits^m$ as being distributed according to $(\sign(\bg \cdot e^1),\dots,\sign(\bg \cdot e^m))$, so our  goal is to show that

\begin{equation} 
\label{eq:humphrey}
\dtv((\sign(\bg \cdot e^1),\dots,\sign(\bg \cdot e^m)),(\sign(\bg \cdot \bg^1),\dots,\sign(\bg \cdot \bg^m))) \leq 0.1.
\end{equation} 

We say that a specific outcome $(g^1,\dots,g^m) \in (\R^n)^m$ of $(\bg^1,\dots,\bg^m) \sim (N(0,I_n))^m$ is \emph{bad} if there is a pair $i\neq j$ such that the normalized inner product ${\frac {|g^i \cdot g^j|}{\|g^i\| \cdot \|g^j\|}}$ is greater than $C\sqrt{{\frac {\log n}n}}$, and otherwise we say that $(g^1,\dots,g^m)$ is \emph{good}. Intuitively, the tuple $(g^1,\dots,g^m)$ is bad if the $m$ vectors $g^1,\dots,g^m$ are not ``pairwise nearly orthogonal''; as we now show, this is very unlikely to happen.
Fix any $1 \leq i \neq j \leq m$; we have that ${\frac {\bg^i}{\|\bg^i\|}}$ and ${\frac {\bg^j}{\|\bg^j\|}}$ are independent uniform vectors on the $n$-dimensional unit sphere $\mathbb{S}^{n-1}$, and so the distribution of  ${\frac {|\bg^i \cdot \bg^j|}{\|\bg^i\| \cdot \|\bg^j\|}} = \left| {\frac {\bg^i}{\|\bg^i\|}} \cdot {\frac {\bg^j}{\|\bg^j\|}}\right|$ is
the same as the distribution of $|\bv_1|$ for a uniform random unit vector $\bv \sim \mathbb{S}^{n-1}$. It is well known (see e.g. Lemma~2.2 of \cite{Ball1997}) that $\Pr_{\bv \sim \mathbb{S}^{n-1}}[|\bv_1| > C \sqrt{\log(n)/n}]$ is at most $1/n^2$ for a suitable choice of the absolute constant $C$.  Thus by a union bound over all $m^2 = o(n)$ many pairs $i \neq j$, we have that 
\[
\Pr[(\bg^1,\dots,\bg^m)\text{~is bad}]\leq {\frac {m^2}{n^2}}<0.05.
\]

Hence to establish (\ref{eq:humphrey}) (and hence \Cref{claim:dtvhalfspace} and \Cref{thm:lb-ltf}) it suffices to prove the following:

\begin{claim} 
\label{claim:hubert}
Fix a good $(g^1,\dots,g^m) \in (\R^n)^m$, where $m = c\sqrt{n}/\log n$.
Then for $\bg \sim N(0,I_n)$ we have that
\begin{equation} \label{eq:mansfield-park}
\dtv((\sign(e^1 \cdot \bg),\dots,\sign(e^m \cdot \bg)),(\sign(g^1 \cdot \bg),\dots,\sign(g^m \cdot \bg))) \leq 0.05.
\end{equation}
\end{claim}
To prove \Cref{claim:hubert} we first observe that (\ref{eq:mansfield-park}) is equivalent to
\begin{equation}\label{eq:pride-and-prejudice}
\dtv((\sign(e^1 \cdot \bg),\dots,\sign(e^m \cdot \bg)),(\sign(g'^1 \cdot \bg),\dots,\sign(g'^m \cdot \bg))) \leq 0.05
\end{equation} 
where we define $g'^i := {\frac {g^i}{\|g^i\|}}$ to be $g^i$ normalized to unit length. Next we recall a recent upper bound on the total variation distance between $n$-dimensional Gaussians due to Devroye, Mehrabian and Reddad:

\begin{theorem} 
[Theorem~1.1 of \cite{DMR20}]  \label{thm:DMR20}
Let $\Sigma_1,\Sigma_2$ be two $m \times m$ positive definite covariance matrices and let $\lambda_1,\dots,\lambda_m$ be the eigenvalues of $\Sigma_1^{-1} \Sigma_2 - I_m$. Then
\[
\dtv(N(0^m,\Sigma_1),N(0^m,\Sigma_2)) \leq {\frac 3 2} \cdot \min\left\{1,\sqrt{\lambda_1^2 + \cdots + \lambda_m^2}\right\} 
\]
\end{theorem}
To apply \Cref{thm:DMR20} we take $\Sigma_1$ to be the identity matrix $I_m$ and $\Sigma_2$ to be the $m \times m$ matrix whose $(i,j)$ entry is $g'^i \cdot g'^j$, so a draw from $N(0,\Sigma_1)$ is distributed as $(e_1 \cdot \bg,\dots,e_m \cdot \bg)$ and a draw from $N(0,\Sigma_2)$ is distributed as
$(g'^1 \cdot \bg,\dots,g'^m \cdot \bg).$  Applying the data processing inequality for total variation distance (see e.g. Proposition~B.1 of \cite{DDOST13}, it follows that the LHS of (\ref{eq:pride-and-prejudice}) is at most $\dtv(N(0^m,\Sigma_1),N(0^m,\Sigma_2))$; we proceed to upper bound the RHS of \Cref{thm:DMR20}.

Let $A$ denote the matrix $\Sigma_1^{-1}\Sigma_2 - I_m$, so $\lambda_1^2,\dots,\lambda_m^2$ are the eigenvalues of $A^2$  and we have $\sqrt{\lambda_1^2 + \cdots + \lambda_m^2} = \sqrt{\tr(A^2))}.$
%(since the sum of eigenvalues of $A^2$ is the trace of $A^2$).
Since each $g'^i$ is a unit vector the matrix $A$ has zero entries on the diagonal, and $A$ has off-diagonal entries that are each at most $C \sqrt{{\frac {\log n} n}}$ in magnitude (because $(g^1,\dots,g^m)$ is good). Hence any diagonal element of $A^2$ is at most ${\frac {C^2 m \log n}{n}}$ in magnitude, and consequently $\tr(A^2) \leq {\frac {C^2 m^2  \log n}{n}}$, which is at most ${\frac 1 {900}}$ for a suitable choice of $m = \Theta(\sqrt{n/\log n}).$ Having $\tr(A^2) \leq {\frac 1 {900}}$ gives that ${\frac 3 2} \cdot \min\left\{1,\sqrt{\lambda_1^2 + \cdots + \lambda_m^2}\right\} \leq 0.05$ as required, and the proofs of \Cref{claim:hubert}, \Cref{claim:dtvhalfspace} and \Cref{thm:lb-ltf} are complete.
\end{proof}

%\href{https://arxiv.org/abs/1810.08693}{the Devroye et al paper}


==> sections/lb-halfspaces.tex <==
%!TEX root = ../distinguishing-writeup.tex

\subsection{A $\tilde{\Omega}(\sqrt{n})$-Sample Lower Bound for Halfspaces} \label{sec:halfspace-lb}

Our first lower bound, \Cref{thm:lb-ltf}, shows that $\Omega(\sqrt{n}/\log n)$ samples are needed to distinguish $N(0,I_n)$ from $N(0,I_n)|_K$ where $K$ is an unknown halfspace whose separating hyperplane passes through the origin. 
Some of the ideas in this lower bound will recur in our lower bound for symmetric ``slabs'' (intersections of two parallel halfspaces) given in \Cref{sec:symmetric-lb}, but by taking advantage of the fact that origin-centered halfspaces are odd functions, we can sidestep some aspects of the argument that arise for slabs; hence we give a self-contained proof for halfspaces below.

\begin{theorem} \label{thm:lb-ltf}
Let $A$ be any algorithm which is given access to samples from an unknown distribution ${\cal D}$ over $\R^n$ and has the following performance guarantee:

\begin{enumerate}

\item If ${\cal D}=N(0,I_n)$, then with probability at least $2/3$ the algorithm outputs ``un-truncated'';

\item If ${\cal D}=N(0,I_n)|_K$ where $K$ is an unknown zero-threshold LTF, then with probability at least $2/3$ the algorithm outputs ``truncated.''

\end{enumerate}
Then $A$ must use at least $\Omega(\sqrt{n}/\log n)$ samples from ${\cal D}$.
\end{theorem}

\begin{proof}
We consider two different distributions, ${\cal D}_1$ and ${\cal D}_2$, each of which is a distribution over sequences of $m$  points in $\R^n$.

\begin{enumerate}

\item A draw of $\overline{\bg}=(\bg^1,\dots,\bg^m)$ from ${\cal D}_1$  is obtained by having each $\bg^i \in \R^n$ be distributed independently according to $N(0,I_n)$.

\item A draw from ${\cal D}_2$ is obtained by independently drawing $\bg,\bg^1,\dots,\bg^m$ from  $N(0,I_n)$ and outputting $(\sign(\bg \cdot \bg^1) \bg^1, \dots, \sign(\bg\cdot \bg^m) \bg^m).$
\end{enumerate}

Observe that a draw from ${\cal D}_2$ is distributed as a sample of $m$  independent draws from $N(0,I_n)|_{\bK}$ where $\bK=\{x \in \R^n: \bg \cdot x \geq 0\}$ is a random zero-threshold LTF defined by a normal vector $\bg$ that is drawn from $N(0,I_n)$ (here is where we are using that any zero-threshold LTF is an odd function). Thus to prove \Cref{thm:lb-ltf} it suffices to show that any algorithm that determines  (with correctness probability at least $2/3$) whether an $m$-element sample came from ${\cal D}_1$ or ${\cal D}_2$ must have $m = \Omega(\sqrt{n}/\log n).$ This is an immediate consequence of the following claim: 

\begin{claim}
\label{claim:dtvhalfspace}
There is a universal constant $c>0$ such that for $m = c \sqrt{n}/\log n$, we have 
$\dtv({\cal D}_1,{\cal D}_2) \leq 0.1.$
\end{claim}

\medskip
\noindent \emph{Proof of \Cref{claim:dtvhalfspace}.}
We first observe that a draw $(\bg^1,\dots,\bg^m) \sim {\cal D}_1$ is distributed identically to $(\bu_1 \bg^1,\dots,
\bu_m \bg^m)$ where each $\bu_i$ is an independent uniform $\bits$ random variable. Next, we observe that
\begin{align} 
\dtv({\cal D}_1,{\cal D}_2) &=
\dtv((\bu_1 \bg^1,\dots,
\bu_m \bg^m),(\sign(\bg \cdot \bg^1) \bg^1, \dots, \sign(\bg\cdot \bg^m) \bg^m))\nonumber \\
&\leq \Ex_{\overline{\bg}}[\dtv((\bu_1\bg^1,\dots,\bu_m\bg^m),(\sign(\bg \cdot \bg^1)\bg^1,\dots,\sign(\bg \cdot \bg^m)\bg^m))] \label{eq:gourd}\\
&= \Ex_{\overline{\bg}}[\dtv((\bu_1,\dots,\bu_m),(\sign(\bg \cdot \bg^1),\dots,\sign(\bg \cdot \bg^m)))] \label{eq:pumpkin}
\end{align}
where $\bu=(\bu_1,\dots,\bu_m)$ is uniform over $\bits^m$; it should be noted that in \Cref{eq:gourd} the randomness in the two random variables whose variation distance is being considered is only over $\bu_1,\dots,\bu_m$ and $\bg$; and the equality between (\ref{eq:gourd}) and (\ref{eq:pumpkin}) holds because the $N(0,I_n)$ distribution has no atoms of mass.   So it remains to bound the expected variation distance between the two $m$-bit strings $\bu$ and $(\sign(\bg \cdot \bg^1),\dots,\sign(\bg \cdot \bg^m))$, where the expectation is over $\overline{\bg}=(\bg^1,\dots,\bg^m)$. We may view a uniform $\bu \sim \bits^m$ as being distributed according to $(\sign(\bg \cdot e^1),\dots,\sign(\bg \cdot e^m))$, so it suffices to show that with probability at least $0.95$ over $\overline{\bg}$, we have
\begin{equation} 
\label{eq:humphrey}
\dtv((\sign(\bg \cdot e^1),\dots,\sign(\bg \cdot e^m)),(\sign(\bg \cdot \bg^1),\dots,\sign(\bg \cdot \bg^m))) \leq 0.05.
\end{equation} 

We say that a specific outcome $(g^1,\dots,g^m) \in (\R^n)^m$ of $(\bg^1,\dots,\bg^m) \sim (N(0,I_n))^m$ is \emph{bad} if there is a pair $i\neq j$ such that the normalized inner product ${\frac {|g^i \cdot g^j|}{\|g^i\| \cdot \|g^j\|}}$ is greater than $C\sqrt{{\frac {\log n}n}}$, and otherwise we say that $(g^1,\dots,g^m)$ is \emph{good}. Intuitively, the tuple $(g^1,\dots,g^m)$ is bad if the $m$ vectors $g^1,\dots,g^m$ are not ``pairwise nearly orthogonal''; as we now show, this is very unlikely to happen.
Fix any $1 \leq i \neq j \leq m$; we have that ${\frac {\bg^i}{\|\bg^i\|}}$ and ${\frac {\bg^j}{\|\bg^j\|}}$ are independent uniform vectors on the $n$-dimensional unit sphere $\mathbb{S}^{n-1}$, and so the distribution of  ${\frac {|\bg^i \cdot \bg^j|}{\|\bg^i\| \cdot \|\bg^j\|}} = \left| {\frac {\bg^i}{\|\bg^i\|}} \cdot {\frac {\bg^j}{\|\bg^j\|}}\right|$ is
the same as the distribution of $|\bv_1|$ for a uniform random unit vector $\bv \sim \mathbb{S}^{n-1}$. It is well known (see e.g. Lemma~2.2 of \cite{Ball1997}) that $\Pr_{\bv \sim \mathbb{S}^{n-1}}[|\bv_1| > C \sqrt{\log(n)/n}]$ is at most $1/n^2$ for a suitable choice of the absolute constant $C$.  Thus by a union bound over all $m^2 = o(n)$ many pairs $i \neq j$, we have that 
\[
\Pr[(\bg^1,\dots,\bg^m)\text{~is bad}]\leq {\frac {m^2}{n^2}}<0.05.
\]

Hence to establish (\ref{eq:humphrey}) (and hence \Cref{claim:dtvhalfspace} and \Cref{thm:lb-ltf}) it suffices to prove the following:

\begin{claim} 
\label{claim:hubert}
Fix a good $(g^1,\dots,g^m) \in (\R^n)^m$, where $m = c\sqrt{n}/\log n$.
Then for $\bg \sim N(0,I_n)$ we have that
\begin{equation} \label{eq:mansfield-park}
\dtv((\sign(e^1 \cdot \bg),\dots,\sign(e^m \cdot \bg)),(\sign(g^1 \cdot \bg),\dots,\sign(g^m \cdot \bg))) \leq 0.05.
\end{equation}
\end{claim}
To prove \Cref{claim:hubert} we first observe that (\ref{eq:mansfield-park}) is equivalent to
\begin{equation}\label{eq:pride-and-prejudice}
\dtv((\sign(e^1 \cdot \bg),\dots,\sign(e^m \cdot \bg)),(\sign(g'^1 \cdot \bg),\dots,\sign(g'^m \cdot \bg))) \leq 0.05
\end{equation} 
where we define $g'^i := {\frac {g^i}{\|g^i\|}}$ to be $g^i$ normalized to unit length. Next we recall a recent upper bound on the total variation distance between $n$-dimensional Gaussians due to Devroye, Mehrabian and Reddad:

\begin{theorem} 
[Theorem~1.1 of \cite{DMR20}]  \label{thm:DMR20}
Let $\Sigma_1,\Sigma_2$ be two $m \times m$ positive definite covariance matrices and let $\lambda_1,\dots,\lambda_m$ be the eigenvalues of $\Sigma_1^{-1} \Sigma_2 - I_m$. Then
\[
\dtv(N(0^m,\Sigma_1),N(0^m,\Sigma_2)) \leq {\frac 3 2} \cdot \min\left\{1,\sqrt{\lambda_1^2 + \cdots + \lambda_m^2}\right\} 
\]
\end{theorem}
To apply \Cref{thm:DMR20} we take $\Sigma_1$ to be the identity matrix $I_m$ and $\Sigma_2$ to be the $m \times m$ matrix whose $(i,j)$ entry is $g'^i \cdot g'^j$, so a draw from $N(0,\Sigma_1)$ is distributed as $(e_1 \cdot \bg,\dots,e_m \cdot \bg)$ and a draw from $N(0,\Sigma_2)$ is distributed as
$(g'^1 \cdot \bg,\dots,g'^m \cdot \bg).$  Applying the data processing inequality for total variation distance (see e.g. Proposition~B.1 of \cite{DDOST13}, it follows that the LHS of (\ref{eq:pride-and-prejudice}) is at most $\dtv(N(0^m,\Sigma_1),N(0^m,\Sigma_2))$; we proceed to upper bound the RHS of \Cref{thm:DMR20}.

Let $A$ denote the matrix $\Sigma_1^{-1}\Sigma_2 - I_m$, so $\lambda_1^2,\dots,\lambda_m^2$ are the eigenvalues of $A^2$  and we have $\sqrt{\lambda_1^2 + \cdots + \lambda_m^2} = \sqrt{\tr(A^2))}.$
%(since the sum of eigenvalues of $A^2$ is the trace of $A^2$).
Since each $g'^i$ is a unit vector the matrix $A$ has zero entries on the diagonal, and $A$ has off-diagonal entries that are each at most $C \sqrt{{\frac {\log n} n}}$ in magnitude (because $(g^1,\dots,g^m)$ is good). Hence any diagonal element of $A^2$ is at most ${\frac {C^2 m \log n}{n}}$ in magnitude, and consequently $\tr(A^2) \leq {\frac {C^2 m^2  \log n}{n}}$, which is at most ${\frac 1 {900}}$ for a suitable choice of $m = \Theta(\sqrt{n/\log n}).$ Having $\tr(A^2) \leq {\frac 1 {900}}$ gives that ${\frac 3 2} \cdot \min\left\{1,\sqrt{\lambda_1^2 + \cdots + \lambda_m^2}\right\} \leq 0.05$ as required, and the proofs of \Cref{claim:hubert}, \Cref{claim:dtvhalfspace} and \Cref{thm:lb-ltf} are complete.
\end{proof}

%\href{https://arxiv.org/abs/1810.08693}{the Devroye et al paper}


==> sections/lb-mixtures.tex <==
%!TEX root = ../distinguishing-writeup.tex

\subsection{An $\Omega(n)$-Sample Lower Bound for Mixtures of Symmetric Convex Sets}
\label{sec:mix-lb}

In this section we show that $\Omega(n)$ samples are needed to distinguish the distribution $N(0,I_n)$ from an unknown distribution in $\Mix$, even if the distribution in $\Mix$ is guaranteed to have variation distance 1 (the largest possible value) from ${\cal N}(0,I_n)$:

\begin{theorem} \label{thm:lb-mixsymm}
Let $A$ be any algorithm which is given access to samples from an unknown distribution ${\cal D}$ and has the following performance guarantee:

\begin{enumerate}

\item If ${\cal D}=N(0,I_n)$, then with probability at least $9/10$ the algorithm outputs ``un-truncated'';

\item If ${\cal D} \in \Mix$ and has $\dtv({\cal D},N(0,1)|_K)=1$ then with probability at least $9/10$ the algorithm outputs ``truncated.''

\end{enumerate}
Then $A$ must use at least $\Omega(n)$ samples from ${\cal D}$.
\end{theorem}

\noindent {\bf Overview.}
\Cref{thm:lb-mixsymm} is the most involved of our lower bounds so we give an overview of the steps of the argument before entering into the actual proof.

\begin{enumerate}

\item We first use \Cref{fact:hellinger-distinguishing} to show that $\Omega(1/\delta)$ samples are required to distinguish $N(0,I_n)$ from $N(0,(1-\delta)I_n)$.  (We will take $\delta:=C/n$ for an absolute constant $C$.)

\item We define a distribution $P$ that is an infinite mixture over distributions $N(0,I_n)|_K$ where each $K$ in the mixture is a symmetric convex set. The mixture $P$ is carefully designed so that $\dtv(N(0,(1-\delta)I_n),P)$ is small, in particular $o(1/n)$ (in fact we will show that it is at most some $\kappa = 1/n^{\omega(1)}$). Consequently by \Cref{fact:dtv-distinguishing}, at least $\Omega(1/\kappa)$ samples are required to distinguish $P$ from $N(0,(1-\delta)I_n)$.

In more detail, each symmetric convex set $K$ in the mixture is the intersection of an $(n-1)$-dimensional hyperplane through the origin with an $n$-dimensional ball.  The radii of these balls are chosen according to a carefully designed distribution, and the directions of the orthogonal vectors to the hyperplanes are (Haar)-uniform random over all possible directions. Consequently $P$ is a radially symmetric distribution; this greatly simplifies the analysis and the proof that indeed $P$ closely approximates the radially symmetric distribution $N(0,(1-\delta)I_n).$

\item Finally, we define a distribution ${\cal F}_P$ over probability distributions $Q$ that are derived from the mixture distribution $P$.  Each distribution $Q$ in the support of ${\cal F}_P$ is a finite mixture of $n^2$ many $N(0,I_n)|_K$ components that are independently chosen from the mixture defining $P$. Since the support of each $Q$ has $n$-dimensional Gaussian volume 0 (since it is contained in the union of $n^2$ many $(n-1)$-dimensional hyperplanes) we have that each $Q$ satisfies $\dtv(Q,N(0,I_n))=1$ as claimed. 

We argue that for a random distribution $\bQ \sim {\cal F}_P$, the variation distance between (the distribution of an i.i.d~sample of $n$ points drawn from $\bQ$) and (the distribution of an i.i.d~sample of $n$ points drawn from $P$) is very small. This implies that $\Omega(n)$ samples are required to distinguish between a random distribution $\bQ$ drawn from ${\cal F}_P$ and $P$ itself.  We note that this high-level approach, of constructing a distribution over distributions from a mixture distribution and using that distribution over distributions for a distinguishing lower bound, is similar in broad outline to the lower bound approach used in \cite{RubinfeldS09}, see Section~4 of that paper. However, the technical arguments required here are entirely different from \cite{RubinfeldS09} (and significantly more involved).

\item
Combining items 1 through 3 above, we get that 
\[
\min\left\{\Omega(1/\delta),\Omega(1/\kappa),\Omega(n)\right\}=\Omega(n)
\]
samples are required to distinguish a random distribution $\bQ$ from $N(0,I_n)$, which gives \Cref{thm:lb-mixsymm}.

\end{enumerate}

We now enter into the formal proof of \Cref{thm:lb-mixsymm}. Suppose that $A$ is an algorithm which receives $cn$ draws from a distribution ${\cal D}$ (where $c>0$ is a suitably small absolute constant) and outputs ``un-truncated'' with probability at least $9/10$ if the distribution ${\cal D}$ is $N(0,I_n)$. We will show that any such algorithm must also output ``un-truncated'' with probability at least $0.8$ when the distribution ${\cal D}$ is some element of $\Mix$.


\begin{claim} [Indistinguishability of $N(0,I_n)$ and $N(0,(1-\delta)I_n)$.] 
\label{claim:two-normals-indistinguishable}
Let $\delta=o(1/\sqrt{n}).$ Any algorithm that distinguishes (with correctness probability at least $9/10$) whether it is being run on samples from $N(0,I_n)$ or $N(0,(1-\delta)I_n)$ must use $\Omega({\frac 1 {\delta^2 n}})$ samples. 
\end{claim}
\begin{proof}
The squared Hellinger distance between two $n$-dimensional normal distributions $P=N(0,\Sigma)$ and $Q=N(0,\Sigma')$ is (\cite{Pardo}, p. 51)
\begin{equation}
\label{eq:pardo}
H^2(P,Q) = 1 - {\frac {\det(\Sigma)^{1/4} \det(\Sigma')^{1/4}}{\det\left({\frac {\Sigma + \Sigma'}{2}}\right)}}.
\end{equation}
In our setting of $\Sigma_1=I_n$ and $\Sigma_2 = (1-\delta)I_n$, this simplifies to
\begin{align*}
1 - {\frac {(1-\delta)^{n/4}}{(1 - {\frac \delta 2})^{n/2}}}
&=1 - {\frac {\exp({\frac n 4}\ln(1-\delta))}{\exp({\frac n 2}\ln(1-{\frac \delta 2}))}}\\
&=1 - {\frac {\exp(-{\frac n 4}(\delta + {\frac {\delta^2} 2} + {\frac {\delta^3} 3} + \cdots)}
{\exp(-{\frac n 2}(-{\frac {\delta} 2} + {\frac {\delta^2} 8} + {\frac {\delta^3} 24} + \cdots)}}\\
&= 1 - \exp\left(- {\frac {\delta^2 n}{16}} + O(\delta^3 n)\right) \tag{since $\delta = o(1/\sqrt{n})$}\\
&= {\frac {\delta^2 n}{16}} \pm O(\delta^3 n),
\end{align*}
from which the claim follows by \Cref{fact:hellinger-distinguishing}.
\end{proof}


We mention that if $\delta$ is chosen too small then it would not be possible to closely approximate $N(0,(1-\delta)I_n)$ with a mixture distribution as we do in \Cref{lem:P-close-to-delta-normal}; on the other hand, $1/\delta$ is a bottleneck on the quantitative lower bound that the overall proof will yield, so we would like $\delta$ to be as small as possible.  We fix $\delta := C/n$ for the rest of the argument for a (large) absolute constant $C$; this choice gives us the following:

\begin{corollary} \label{cor:two-normals}
The algorithm $A$ must output ``un-truncated'' with probability at least $89/100$ if it is run on $cn$ draws from $N(0,(1-\delta)I_n)$.
\end{corollary}

\subsubsection{The Mixture Distribution $P$}
\label{subsubsec:mixture-lb}
%\paragraph{The Mixture Distribution $P$.}  
We now describe the mixture distribution $P$; its construction and the analysis establishing \Cref{lem:P-close-to-delta-normal} are the main part of the proof of \Cref{thm:lb-mixsymm}. In particular, we will approximate $N(0,(1-\delta)I_n)$ with a mixture $P$ over distributions $N(0,I_n)|_K$ where each $K$ is a symmetric convex body. 

\begin{remark}
We define a parameter $\delta'$ to satisfy $1-\delta = (1+\delta')^{-1}$, so $N(0,(1-\delta)I_n)$ is the same as $N(0,(1+\delta')^{-1}I_n)$; this simplifies notation in our analysis below. We observe that like $\delta$, the value $\delta'$ is $C/n$ (for a different large absolute constant $C$).
\end{remark}

We now describe the mixture distribution $P$. The distribution over the convex bodies $\bK$ defining the mixture is as follows:  a random convex body $\bK$ from the distribution is the intersection of an origin-centered $(n-1)$-dimensional hyperplane with a ball of radius $\sqrt{\bR}$, where we choose the direction of the hyperplane according to the Haar measure on $S^{n-1}$, and we draw $\bR \in [0,\infty)$ with probability $\lambda(\bR)$ (defined below in \Cref{def:lambdaR}).  

\begin{remark} \label{rem:reassurance}
The attentive reader may notice that the sets $\bK$ defined above have
$\vol(\bK)=0$, and thus $N(0,I_n)|_{\bK}$ is the standard normal distribution conditioned on an event of measure zero.
For this to be a well defined operation (see e.g. \cite{BorelKolmogorov:wikipedia}),  we need to specify how our measure-zero sets are obtained as the limit of a sequence of sets of positive measure.
The limiting process we use for a set $K = H \cap \Ball(\sqrt{R})$ (where $H=H_0$ is the hyperplane $\{x \in \R^n: v \cdot x = 0\}$ is taking a sequence of slabs $H_\eps = \{x: |v \cdot x| \leq \eps\}$ and letting $\eps \to 0$). In the limit the distribution induced for $N(0,I_n)|_H$ is a symmetric distribution restricted to $H$, where the probability assigned to points of squared Euclidean distance $x$ from the origin is $\chi^2(n-1,1)(x)$.  This will be used in \Cref{prop:tv-1-dimensional} below.
\end{remark}

Recall that for $\bx\sim N(0,I_n)$, the random variable $\|\bx\|^2$ is distributed according to a $\chi^2(n)$ distribution. In particular, a draw $\bx\sim N(0,I_n)$ can be viewed as 
\begin{enumerate}
	\item First drawing $\bv\sim S^{n-1}$ according to the Haar measure, then
	\item Drawing $\bX\sim\chi^2(n)$;
\end{enumerate}
and then outputting $\bv\cdot\sqrt{\bX}$. A draw from $N(0,(1+\delta')^{-1}I_n)$ can be similarly viewed, except with $\bX$ drawn from a \emph{scaled} $\chi^2(n)$ distribution. For convenience, we introduce the following notation.
 
\begin{notation}
	We will write $\chi^2(n, \sigma^2)$ to denote the distribution of $\|\bx\|^2$ for $\bx\sim N(0,\sigma^2 I_n)$. We will also write $\chi^2(n,\sigma^2)|_R$ for the truncated distribution $\chi^2(n,\sigma^2)|_{[0,R]}$.
\end{notation}

It is easy to check that if $\bX\sim\chi^2(n, \sigma^2)$, then $\bX/\sigma^2 \sim \chi^2(n,1) = \chi^2(n)$. In particular, we have the following expression for the density of $\bX$:

\begin{fact} \label{fact:chi-pdf}
	The density of the $\chi^2(n,\sigma^2)$ distribution is
	\[\chi^2(n, \sigma^2)(x) = \frac{1}{2^{n/2}\Gamma\pbra{\frac{n}{2}}}\pbra{\frac{x}{\sigma^2}}^{n/2 - 1} e^{-x/2\sigma^2}.\]
\end{fact}


\begin{notation}
	We will write $p(\cdot)$ to denote the density of $\target$, $q_R(\cdot)$ for the density of $\ballsR$, and $\psi(R)$ for the c.d.f. of $\chi^2(n-1,1)$, i.e. we have 
	\[\psi(R) := \Pr\sbra{\chi^2(n-1,1) \leq R}.\] 
\end{notation}

In particular, the following is immediate from \Cref{fact:chi-pdf}:
\begin{equation} \label{eq:p}
	p(x) = \frac{(1+\delta')^{n/2 -1} x^{n/2-1} e^{-(1+\delta')x/2}}{2^{n/2}\Gamma\pbra{\frac{n}{2}}},
\end{equation}
\begin{equation} \label{eq:qR}
	q_R(x) = \frac{x^{(n-1)/2 - 1}e^{-x/2}}{2^{(n-1)/2}\Gamma\pbra{\frac{n-1}{2}}} \cdot \frac{\Indicator(x\leq R)}{\psi(R)}.
\end{equation}
Note that a draw from the mixture $P$ can thus be viewed as 
\begin{enumerate}
	\item First drawing $\bv\sim S^{n-1}$ according to the Haar measure, then
	\item Drawing $\bY\sim S$;
\end{enumerate}
and outputting $\bv\cdot\sqrt{\bY}$.  Defining the univariate distribution $S$ over $[0,\infty)$ whose density is
\begin{equation}
S(x) = \int_{R}\lambda(R)\cdot q_R(x)\,dR,
\label{eq:eggs}
\end{equation}
by rotational symmetry, we have the following:

\begin{proposition} \label{prop:tv-1-dimensional}
	We have 
	\[\dtv\pbra{P, N(0,(1+\delta')^{-1}I_n)} = \dtv\pbra{S, \target}.\]
\end{proposition}

We thus want to come up with mixing weights $\lambda(R)$ such that the total variation distance between the univariate distributions $p$ and $S$ is small.
It will turn out by our choice of $\lambda(R)$ below that in fact $S(x)$ will not just approximate $p(x)$, but will in fact be \emph{exactly} equal to $p(x)$ for all $x \geq a^\ast$ for a carefully chosen $a^\ast$. In particular, our choice of $\lambda(R)$ (see \Cref{def:lambdaR}) will ensure that:
\begin{enumerate}
	\item $S(a^\ast) = p(a^\ast)$; and
	\item $S'(x) = p'(x)$ for all $x\geq a^\ast$.
\end{enumerate}

We start by simplifying the expressions for $S(\cdot)$ and $p(\cdot)$ (cf. \Cref{eq:p,eq:qR}). Indeed, having $S(x) = p(x)$ is equivalent to having 
\begin{align*}
\frac{x^{(n-1)/2 - 1}e^{-x/2}}{2^{(n-1)/2}\Gamma\pbra{\frac{n-1}{2}}}\int_R \frac{\lambda(R)}{\psi(R)}\cdot \Indicator(x \leq R) \,dR &= \frac{(1+\delta')^{n/2 -1} x^{n/2-1} e^{-(1+\delta')x/2}}{2^{n/2}\Gamma\pbra{\frac{n}{2}}},
\end{align*}
which can be rearranged to get 
\begin{equation} \label{eq:thing-we-diff}
\int_{x}^\infty \frac{\lambda(R)}{\psi(R)}\,dR = \frac{\Gamma\pbra{\frac{n-1}{2}}}{\sqrt{2}\cdot\Gamma\pbra{\frac{n}{2}}}\cdot(1+\delta')^{n/2 - 1}\cdot\pbra{\sqrt{x}e^{-\delta' x/2}}.
\end{equation}
Next, we ensure that that $S'(x) = p'(x)$, i.e. the second item above, before choosing $a^\ast$. Differentiating both sides of \Cref{eq:thing-we-diff}, via the fundamental theorem of calculus we get that 
\begin{equation} \label{eq:first-lambda-formula}
\frac{\lambda(x)}{\psi(x)} = \frac{\Gamma\pbra{\frac{n-1}{2}}}{\sqrt{2}\cdot\Gamma\pbra{\frac{n}{2}}}\cdot(1+\delta')^{n/2 - 1}\cdot e^{-\delta' x/2}\pbra{\frac{\delta' x - 1}{2\sqrt{x}}}
\end{equation}
This suggests taking 
\[\lambda(x) := \psi(x) \cdot (\text{RHS of \Cref{eq:first-lambda-formula}}),\] 
but this clearly does not result in a valid distribution over $R$ as $\lambda(x)$ will be negative for $x < 1/\delta'$; see \Cref{fig:lambda}. However, as the following claim shows, for the above choice of $\lambda$ we do have that $\int_0^{\infty} \lambda(R) \,dR = 1$:

\begin{claim} \label{claim:integral-is-1}
	For $\lambda(R)$ defined as in \Cref{eq:first-lambda-formula}, we have
	\[\int_R \lambda(R)\,dR = 1.\]
\end{claim}

\begin{proof}
	We have 
	\begin{align*}
		\int_R \lambda(R)\,dR &= \frac{\Gamma\pbra{\frac{n-1}{2}}}{\sqrt{2}\cdot\Gamma\pbra{\frac{n}{2}}}\cdot(1+\delta')^{n/2 - 1} \int_R \underbrace{e^{-\delta' R/2}\pbra{\frac{\delta' R - 1}{2\sqrt{R}}}}_{=:v'(R)}\psi(R)\, dR\\
		\intertext{for $v(x) := -\sqrt{x}e^{-\delta' x/2}$; integrating by parts then gives us}
		&= \frac{\Gamma\pbra{\frac{n-1}{2}}}{\sqrt{2}\cdot\Gamma\pbra{\frac{n}{2}}}\cdot(1+\delta')^{n/2 - 1} 
		\pbra{\sbra{v(R)\psi(R)}_{0}^\infty - \int_R v(R)\psi'(R)\,dR}.\\
			\intertext{Note, however, that $\lim_{x\to\infty} v(x) = 0$ and $\psi(0) = 0$. We also have that $\psi'(R) = \balls(R)$, and so using \Cref{fact:chi-pdf} the above simplifies to}
		&= \frac{\Gamma\pbra{\frac{n-1}{2}}}{\sqrt{2}\cdot\Gamma\pbra{\frac{n}{2}}}\cdot(1+\delta')^{n/2 - 1} \int_R \sqrt{R}e^{-\delta' R/2} \cdot \frac{R^{(n-1)/2 - 1} e^{-R/2}}{2^{(n-1)/2}\Gamma\pbra{\frac{n-1}{2}}}\, dR\\
		&= \frac{1}{2^{n/2}\cdot\Gamma\pbra{\frac{n}{2}}}\cdot(1+\delta')^{n/2 - 1} \int_R R^{n/2 - 1} e^{-(1+\delta')R/2}\,dR\\
		&= \int_R p(R)\,dR\\
		&= 1,
	\end{align*}
	completing the proof.
\end{proof}



%%%%%%%%%%%%%% another fig %%%%%%%%%%%%%%%%
\input{sections/curvy}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\Cref{claim:integral-is-1} and the fact that $\lambda(R) < 0$ iff $R<1/\delta$ together suggest a natural way to obtain a valid distribution over $\R$ from $\{\lambda(R)\}$. This is by truncating the support of $\lambda(R)$ to $[a^\ast, \infty)$, where we take
\begin{equation} \label{eq:a-ast}
	a^\ast > \frac{1}{\delta'} \qquad\text{such that} \qquad -\int_{0}^{1/\delta'} \lambda(R)\,dR = \int_{1/\delta'}^{a^\ast} \lambda(R)\,dR.
\end{equation} 
(See also \Cref{fig:lambda}.) We thus have the following:

\begin{definition}[Mixing weights]
\label{def:lambdaR}
	For $R\geq0$, we define the mixing weight $\lambda(R)$ to be 
	\[\lambda(R) := 
	\begin{cases}
		0 & R < a^\ast \\
		\frac{\Gamma\pbra{\frac{n-1}{2}}}{\sqrt{2}\cdot\Gamma\pbra{\frac{n}{2}}}\cdot(1+\delta')^{n/2 - 1}\cdot e^{-\delta' R/2}\pbra{\frac{\delta' R - 1}{2\sqrt{R}}}\cdot \psi(R)
 & R\geq a^\ast
	\end{cases}.\]	
\end{definition}

By construction, we have that $\lambda_R \geq 0$ for all $R$, and that $\int \lambda_R\, dR = 1$. Furthermore, for this choice of $\lambda(\cdot)$, we have from \Cref{eq:thing-we-diff,eq:first-lambda-formula} that $S'(x) = p'(x)$ for all $x\geq a^\ast$. We will now show that we also have $S(a^\ast) = p(a^\ast)$, establishing the first item.

\begin{claim}
	For $a^\ast$ as in \Cref{eq:a-ast}, we have $S(a^\ast) = p(a^\ast)$.
\end{claim}

\begin{proof}
	The mass at $a^\ast$ under $S$ is given by 
	\begin{align*}
		S(a^\ast) &= \int_R \lambda(R)q_R(a^\ast)\,dR\\
		&= \frac{1}{2^{n/2}\Gamma\pbra{\frac{n}{2}}}\cdot(1+\delta')^{n/2 - 1}\int_R e^{-\delta' R/2}\pbra{\frac{\delta' R - 1}{2\sqrt{R}}} e^{-a^\ast/2}\cdot (a^\ast)^{(n-1)/2 -1}\Indicator(a^\ast\leq R)\, dR\\
		&= \frac{(1+\delta')^{n/2 - 1}e^{-a^\ast/2}\cdot (a^\ast)^{(n-1)/2 -1}}{2^{n/2}\Gamma\pbra{\frac{n}{2}}}{\int_{a^\ast}^\infty e^{-\delta' R/2}\pbra{\frac{\delta' R - 1}{2\sqrt{R}}}\,dR}.
	\end{align*}
	As before, integration by parts gives 
	\[\int_{a^\ast}^\infty e^{-\delta' R/2}\pbra{\frac{\delta' R - 1}{2\sqrt{R}}}\,dR = e^{-\delta' a^\ast/2}\sqrt{a^\ast},\] 
	and so we have 
	\[S(a^\ast) = \frac{(1+\delta')^{n/2 - 1}e^{-(1+\delta')a^\ast/2}\cdot (a^\ast)^{n/2 -1}}{2^{n/2}\Gamma\pbra{\frac{n}{2}}} = p(a^\ast),\]
	completing the proof. 
\end{proof}

We finally turn to establishing the closeness of $P$ and $N(0, (1+\delta')^{-1}I_n)$ (recall that by our choice of $\delta'=C/n$ we have that $N(0,(1+\delta')^{-1}I_n)$ is the same as $N(0,(1-\delta)I_n)$).
 
\begin{lemma}[Closeness of $P$ and $N(0,(1+\delta')^{-1}I_n)$] \label{lem:P-close-to-delta-normal}
$\dtv(P,N(0,(1+\delta')^{-1}I_n)) \leq \kappa := 1/n^{\omega(1)}.$
\end{lemma}

\begin{proof}
Note that by \Cref{prop:tv-1-dimensional}, it suffices to show that 
\[\dtv\pbra{S, \target} \leq \kappa.\]
However, by our construction of $S$ above (see also \Cref{fig:lambda}), we have that $S(x) = p(x)$ for all $x \geq a^\ast$, and so 
\begin{equation} \label{eq:almost-done}
	\dtv\pbra{S, \target} \leq \Prx_{\bX\sim\target}\sbra{\bX\leq a^\ast};
\end{equation}
hence to prove \Cref{lem:P-close-to-delta-normal} it suffices to show that the RHS of \Cref{eq:almost-done} is $1/n^{\omega(1)}$.
	
Recall from \Cref{eq:a-ast} that $a^\ast > 1/\delta' = n/C$ for some absolute constant $C$, and was chosen such that 
	\begin{equation}
	-\int_0^{1/\delta'} \lambda(R)\,dR = \int_{1/\delta'}^{a^\ast}\lambda(R)\,dR \label{eq:dickens}
	\end{equation}
	where $\lambda(R)$ is given by \Cref{eq:first-lambda-formula}. In particular, for our choice of $\delta'$ we have
	\[\lambda(R) = \underbrace{\frac{\Gamma\pbra{\frac{n-1}{2}}}{\sqrt{2}\cdot\Gamma\pbra{\frac{n}{2}}}\cdot(1+\delta')^{n/2 - 1}}_{=\Theta\pbra{\frac{1}{\sqrt{n}}}} e^{-\delta' R/2}\pbra{\frac{\delta' R - 1}{2\sqrt{R}}}\cdot\psi(R).\]
	For $R \leq n/C$ for large enough $C$, we thus have (using standard tail bounds on the $\chi^2$ distribution, cf. \Cref{lem:johnstone}) that $|\lambda(R)| = O(e^{-cn})$. Hence by \Cref{eq:dickens} we get that
	\begin{equation} \label{eq:thing-to-contradict}
		\int_{1/\delta'}^{a^\ast} \lambda(R)\,dR \leq \frac{1}{\delta'}\cdot O(e^{-cn}) = \frac{n}{C'e^{c'n}}
	\end{equation}
	where $c'$ and $C'$ are absolute constants. 
	We will establish the following claim:
	
	\begin{claim} \label{claim:aast-not-too-big}
	$a^\ast \leq n - n^{3/4}.$
	\end{claim}
	
	Given \Cref{claim:aast-not-too-big}, we have that the RHS of \Cref{eq:almost-done} is
	$\Pr_{\bX \sim \chi^2(n,1)}[\bX \leq (n-n^{3/4})(1+\delta')]$, which is at most $2^{-\Theta(n^{1/2})}$ by \Cref{lem:johnstone}, which gives \Cref{lem:P-close-to-delta-normal}. 
	
	To establish \Cref{claim:aast-not-too-big}, suppose (for the sake of contradiction) that $a^\ast \geq n - n^{3/4}.$ For each $x \in [n-2n^{3/4},n-n^{3/4}]$ we have  that
	\begin{align}
	\chi^2(n,1)(x) &= \frac{1}{2^{n/2}\Gamma\pbra{\frac{n}{2}}}x^{n/2 - 1} e^{-x/2}  \tag{by \Cref{fact:chi-pdf}} \nonumber \\
	&\geq \frac{1}{2^{n/2} \lfloor {\frac n 2 - 1} \rfloor !}\pbra{n-2n^{3/4}}^{n/2 - 1} e^{-(n-2n^{3/4})/2}
	\label{eq:unim}\\
	&\geq {\frac 1 {\poly(n) \cdot 2^{n/2} \cdot \left({\frac n {2e}}\right)^{n/2 - 1}}}   n^{n/2 - 1} \left(
	1 - {\frac 2 {n^{1/4}}}\right)^{n/2 - 1} e^{-(n-2n^{3/4})/2} \nonumber\\
	&= {\frac 1 {\poly(n)}} \left(1 - {\frac 2 {n^{1/4}}}\right)^{n/2 - 1} e^{n^{3/4}} \nonumber\\
	&\geq {\frac 1 {\poly(n)}} e^{-2n^{3/4}} e^{n^{3/4}} \tag{using $1-x \geq e^{-2x}$ for $0<x<0.1$}
	\nonumber \\
	& \geq e^{-1.5n^{3/4}} \nonumber.
	\end{align}
where (\ref{eq:unim}) is by unimodality of the $\chi^2(n,1)$ distribution and the fact that its mode is $n-2 > n-n^{3/4}$.
	Hence 
	\[
	\Prx_{\bX \sim \chi^2(n,1)}[\bX \leq n - 1.5n^{3/4}] \geq 
	\Prx_{\bX \sim \chi^2(n,1)}[\bX \in [n-2n^{3/4}, n - 1.5n^{3/4}] \geq 
	(1/2)n^{3/4} \cdot e^{-1.5n^{3/4}},
	\]
	which implies that
	$\Pr_{\bX \sim \chi^2\left(n,(1+\delta')^{-1}\right)}[\bX \leq n - n^{3/4}] \geq (1/2)n^{3/4} \cdot e^{-1.5n^{3/4}}$.
		Comparing with \Cref{eq:thing-to-contradict} this gives \Cref{claim:aast-not-too-big}, which in turn completes the proof of \Cref{lem:P-close-to-delta-normal}.	
%	we then have $[n-2\log(n)\sqrt{n},\geq n - \log(n)\sqrt{n}] =: T \sse [1/\delta', a^\ast]$. For $R \in T$, we have 
%	\[e^{-\delta' R / 2} = \Theta(1).\]
%	\red{We also for $R \in T$ that $\lambda(R) \geq \frac{1}{2^{O\pbra{\log^2(n)}}}$, and so 
%	\[\int_{1/\delta'}^{a^\ast} \lambda(R)\,dR \geq \log(n)\sqrt{n} \cdot \frac{1}{\mathrm{quasipoly}(n)} \gg \frac{n}{C'e^{c'n}},\]
%	contradicting \Cref{eq:thing-to-contradict}.}\snote{I feel like I am being stupid here! Is there a known lower bound on $\psi(R)$? Anti-concentration for norm of a Gaussian feels like it should be known, but I couldn't find anything meaningful. (Carbery-Wright doesn't seem to give anything meaningful here?) I think the thing in red is true---in fact, maybe something stronger is true---via the Cramer-Chernoff method, see e.g. the first centered math block \href{https://sites.stat.washington.edu/jaw/COURSES/580s/581/HO/Chernoff-Cramer.pdf}{here}.}
%	
%	We thus have that $a^\ast \leq n - \log(n)\sqrt{n}$. Combining this with \Cref{eq:almost-done}, we get that 
%	\[\dtv\pbra{S, \target} \leq \frac{1}{\exp\pbra{O(\log^2(n))}},\]
%	completing the proof. 
\end{proof}

Combining \Cref{lem:P-close-to-delta-normal} and \Cref{cor:two-normals} we obtain the following:

\begin{corollary} \label{cor:P-close-to-original-normal}
The algorithm $A$ must output ``un-truncated'' with probability at least $88/100$ if it is run on $cn$ draws from $P$.
\end{corollary}


\subsubsection{The Distribution ${\cal F}_P$} 

We now describe the distribution ${\cal F}_P$, which is a distribution over distributions $Q$ over $\R^n$. A draw of a distribution $\bQ$ from ${\cal F}_P$ is obtained as follows: $\bQ$ is a uniform mixture of $n^2$ many distributions, where the $i$-th distribution in the mixture is $N(0,I_n)|_{\bK_i}$, where each $\bK_i$ is i.i.d.~drawn from the distribution ${\cal K}$.

It is clear that each distribution $Q$ in the support of ${\cal F}_P$ has $\vol(\supp(Q))=0$ and hence $\dtv(N(0,I_n),Q)=1.$
Let $\bS$ be a random variable which takes values in $(\R^n)^{cn}$, where a draw from $\bS$ is obtained by making $cn$ independent draws from $P$.
Let $\bS'$ be a random variable which also takes values in $(\R^n)^{cn}$, where a draw from $\bS'$ is obtained by (i) first randomly drawing a $\bQ \sim {\cal F}_P$, and then (ii) making $cn$ independent draws from $\bQ$.

\begin{claim} \label{claim:S-versus-S'}
$\dtv(\bS,\bS') \leq {\frac 1 {100}}.$
\end{claim}
\begin{proof}
The idea is similar to the proof of Claim~7 of \cite{RubinfeldS09}; for completeness we recall the simple argument here. By the Birthday Paradox, with probability at least $99/100$ the $cn$ independent draws from $\bQ$ come from $N(0,I_n)|_{\bK_{i_1}},
\dots,N(0,I_n)|_{\bK_{i_{cn}}}$ such that $i_{1},\dots,i_{cn}$ are $cn$ distinct values from $[n^2]$. If this happens then the distribution of $\bS'$ is identical to the distribution of $\bS$, since in both cases each of the $cn$ vectors in $\R^n$ is independently drawn by first selecting a component $\bK \sim {\cal K}$ and then making a draw from $N(0,I_n)|_{\bK}.$ This gives the claim.
\end{proof}

From \Cref{claim:S-versus-S'} and \Cref{cor:P-close-to-original-normal} we obtain the following, which completes the proof of \Cref{thm:lb-mixsymm}:

\begin{corollary} \label{cor:end}
The algorithm $A$ must output ``un-truncated'' with probability at least $87/100$ if it is run on $cn$ draws from $P$.
\end{corollary}


==> sections/lb-slabs-garbage.tex <==
%!TEX root = ../distinguishing-writeup.tex

\subsection{ A $\tilde{\Omega}(\sqrt{n})$-Sample Lower Bound for Symmetric Convex Bodies (Slabs)} \label{sec:symmetric-lb}

Given a unit vector $v \in \mathbb{S}^{n-1}$ and a positive value $r>0$, we say that the \emph{symmetric slab of width $2r$ in direction $v$} is the symmetric convex set $\Slab_{v,r} := \{x \in \R^n: |v \cdot x| \leq r\}.$  
Our second lower bound shows that $\Omega(\sqrt{n}/\log n)$ samples are needed to distinguish $N(0,I_n)$ from $N(0,I_n)|_K$ where $K$ is an unknown symmetric slab that is promised to have volume roughly $1/2$:

\begin{theorem} \label{thm:lb-slab}
Let $A$ be any algorithm which is given access to samples from an unknown distribution ${\cal D}$ and has the following performance guarantee:

\begin{enumerate}

\item If ${\cal D}=N(0,I_n)$, then with probability at least $9/10$ the algorithm outputs ``un-truncated'';

\item If ${\cal D}=N(0,I_n)|_K$ where $K$ is an unknown symmetric slab with $\vol(K) \in [0.49,0.51]$, then with probability at least $9/10$ the algorithm outputs ``truncated.''

\end{enumerate}
Then $A$ must use at least $\Omega(\sqrt{n}/\log n)$ samples from ${\cal D}$.
\end{theorem}


\begin{proof}
Let $\psi: \R \to \{0,1\}$ be the function $\psi(t) = \Indicator[|t| \leq c]$ where $c \approx 0.68$ is the real number satisfying $\Pr_{\bg \sim N(0,1)}[|\bg| \leq c]=1/2.$
We define a distribution ${\cal K}$ over symmetric slabs as follows: to draw a symmetric slab $\bK \sim {\cal K}$, first draw a standard Normal vector $\bg \sim N(0,I_n)$, and let $\bK=\bK_{\bg}$ be the symmetric slab $\bK = \{x \in \R^n: \psi({\frac {\bg}{\sqrt{n}}} \cdot x)=1\}.$

We observe that given a particular outcome $g$ of $\bg$, the width of the slab $K=\bK_{g}$ is ${\frac {2c \sqrt{n}}{\|g\|}}$, and hence the volume $\vol(K)$ is $\Pr_{\bx \sim N(0,1)}[|\bx| < {\frac {c \sqrt{n}}{\|g\|}}].$ Standard tail bounds on the chi-distribution (which is the distribution of $\|\bg\|$ for $\bg \sim N(0,I_n)$) imply that $\Pr_{\bK \sim {\cal K}}[\vol(\bK) \notin [0.49,0.51]]$ is extremely small, in particular at most $1/n^{\omega(1)}$. 
Hence to prove \Cref{thm:lb-slab}, it suffices to prove an $\Omega(\sqrt{n} / \log n)$ lower bound on the sample complexity of any algorithm $A$ that outputs ``un-truncated'' with probability at least $9/10$ if it is given samples from $N(0,I_n)$ and outputs ``truncated'' with probability at least $91/100$ if it is given samples from $N(0,I_n)|_{\bK}$ where $\bK \sim {\cal K}$. We do this in the rest of the proof.

We consider two different distributions, ${\cal D}_1$ and ${\cal D}_2$, each of which is a distribution over sequences of $m=c\sqrt{n} / \log n$  points in $\R^n$:

\begin{enumerate}

\item A draw of $\overline{\bx}=(\bx^1,\dots,\bx^{m})$ from ${\cal D}_1$  is obtained by having each $\bx^i \in \R^n$ be distributed independently according to $N(0,I_n)$.

\item A draw of $\overline{\bx}=(\bx^1,\dots,\bx^{m})$ from ${\cal D}_2$ is obtained by drawing (once and for all) a set $\bK=\bK_{\bg} \sim {\cal K}$ (so $\bg \sim N(0,I_n)$) and having each $\bx^i$ be distributed independently according to $N(0,I_n)|_{\bK}$, i.e. each $\bx^i$ is drawn from $N(0,I_n)$ conditioned on  satisfying $\psi({\frac {\bg}{\sqrt{n}}} \cdot x)=1.$
\end{enumerate}

We further define two more distributions ${\cal D}'_1$ and ${\cal D}'_2$, each of which is a distribution over sequences of $3m$ points in $\R^n$:

\begin{enumerate}

\item A draw of $\overline{\bx}=(\bx^1,\dots,\bx^{3m})$ from ${\cal D}'_1$ is obtained as follows: $\bx^i$ is taken to be $\bb_i \bg^i$ where each $\bb_i$ is an independent uniform draw from $\zo$ and each $\bg^i$ is an independent draw from $N(0,I_n)$.

\item A draw of $\overline{\bz}=(\bz^1,\dots,\bz^{3m})$ from ${\cal D}'_2$ is obtained as follows:  once and for all draw $\bg \sim N(0,I_n)$, and take $\bz^i$ to be $\bg^i \cdot \psi({\frac {\bg}{\sqrt{n}}} \cdot \bg^i)$ where each $\bg^i$ is an independent draw from $N(0,I_n)$.

\end{enumerate}


Suppose that algorithm $A$ successfully distinguishes between ${\cal D}_1$ and ${\cal D}_2$, i.e. it outputs ``un-truncated'' with probability at least 9/10 when run on a draw from ${\cal D}_1$ and outputs ``truncated'' with probability at least 91/100 when run on a draw from ${\cal D}_2.$
We claim that then there is an algorithm $A'$ which successfully distinguishes between ${\cal D}'_1$ and ${\cal D}'_2$, i.e. it outputs ``un-truncated'' with probability at least 89/100 when run on a draw from ${\cal D}'_1$ (recall that this is a sequence of $3m$ points in $\R^n$) and outputs ``truncated'' with probability at least 90/100 when run on a draw from ${\cal D}'_2.$  This algorithm $A'$ simply takes the first $m$ nonzero points in its $3m$-point input sequence and uses them as input to $A$.  (We may suppose that $A'$ fails if there are fewer than $m$ nonzero points in the $3m$-point sample; it is easy to see that whether the input to $A'$ is drawn from ${\cal D}'_1$ or ${\cal D}'_2$, the probability of failure is at most $1/n^{\omega(1)}$ and hence is negligible.)  If the input sequence is a draw from ${\cal D}'_1$ then the input that $A'$ gives to $A$ is distributed according to ${\cal D}_1$, and if the input is a draw from ${\cal D}'_2$ then the input sequence that $A'$ gives to $A$ is distributed according to ${\cal D}_2$ (note that we may safely ignore the probability-0 event that some $\bg^i$ drawn from $N(0,I_n)$ is the zero vector).

Given the above claim, to prove \Cref{thm:lb-slab} it suffices to show that any algorithm $A'$ with the performance guarantee described above must have $3m = \Omega(\sqrt{n}/\log n).$  This follows from the statement
\begin{equation}
\label{eq:dtvprimes}
\text{If $m = c \sqrt{n}/\log n$, then~~~~}\dtv({\cal D}'_1,{\cal D}'_2) \leq 0.01.
\end{equation}
The rest of the proof establishes (\ref{eq:dtvprimes}).

Consider a coupling of the two distributions ${\cal D}'_1$ and ${\cal D}'_2$ as follows. A draw from the joint coupled distribution of $({\cal D}'_1,{\cal D}'_2)$ is generated in the following way:

\begin{itemize}

\item Let $(\bb_1,\dots,\bb_{3m})$ be a uniform random string from $\zo^{3m}$. 
\item Let $\bg, \bg^1,\dots,\bg^m$ be $3m+1$ independent draws from $N(0,I_n).$
\item The draw from the joint coupled distribution is $(\overline{\bx},\overline{\bz})$ where
\[
\text{for each $i =1,\dots,3m$,~~~}\bx^i = \bb_i \bg^i \quad \text{and}\quad
 \bz^i=\psi\left({\frac {\bg}{\sqrt{n}}} \cdot \bg^i\right) \bg^i .
\]
\end{itemize}
It is easily verified that this is indeed a valid coupling of ${\cal D}'_1$ and ${\cal D}'_2$.
We thus have
\begin{align}
\dtv({\cal D}'_1,{\cal D}'_2) 
&= \dtv((\bx^1,\dots,\bx^{3m}),(\bz^1,\dots,\bz^{3m})) \nonumber\\
&=\dtv\left((\bb_1\bg^1,\dots,\bb_{3m}\bg^{3m}),
\left(
\psi\left({\frac {\bg}{\sqrt{n}}} \cdot \bg^1\right) \bg^1,
\psi\left({\frac {\bg}{\sqrt{n}}} \cdot \bg^{3m}\right) \bg^{3m}
 \right)\right) \nonumber\\
 &\leq \dtv\left((\bb_1,\dots,\bb_{3m}),\left(\psi\left({\frac {\bg}{\sqrt{n}}} \cdot \bg^1\right),
 \dots, \psi\left({\frac {\bg}{\sqrt{n}}} \cdot \bg^{3m}\right)\right)\right) \label{eq:ham}
\end{align}
where the inequality uses the coupling described above. 
It remains to show that if $m = c \sqrt{n}/\log n$ then $(\ref{eq:ham}) \leq 0.01.$

We observe that for $\bg \sim N(0,I_n)$, we have that $\Pr[\psi(e_i \cdot \bg)=1]=\Pr[\psi(\bg_i)=1]=1/2$. Since the random variables $\{\bg_i\}_{i=1,\dots,3m}$ are independent, we have that the joint distribution of $(\bb_1,\dots,\bb_{3m})$ is identical to the joint distribution of $(\psi(e_1 \cdot \bg),\dots,\psi(e_{3m} \cdot \bg))$, namely, both distributions are uniform over $\zo^{3m}.$ Thus we have that
\begin{equation}
\label{eq:cheese}
(\ref{eq:ham}) = \dtv\left((\psi(e_1 \cdot \bg),\dots,\psi(e_{3m} \cdot \bg)),
\left(\psi\left({\frac {\bg^1}{\sqrt{n}}} \cdot \bg\right),
 \dots, \psi\left({\frac {\bg^{3m}}{\sqrt{n}}} \cdot \bg\right)\right)\right).
 \end{equation}
The rest of the argument proceeds similarly to the proof of \Cref{claim:dtvhalfspace} following (\ref{eq:humphrey}): briefly, for most outcomes $(g^1,\dots,g^{3m})$ of $\bg^1,\dots,\bg^{3m}$, the covariance structure of the two $3m$-dimensional Gaussians $(e_1 \cdot \bg,\dots,e_{3m} \cdot \bg)$ and $({\frac {g^1}{\sqrt{n}}} \cdot \bg,\dots,{\frac {g^{3m}}{\sqrt{n}}} \cdot \bg)$ are similar enough that we can bound the variation distance between those two Gaussians, which implies a bound on the variation distance between $(\psi(e_1 \cdot \bg),\dots,\psi(e_{3m} \cdot \bg))$ and $\left(\psi\left({\frac {g^1}{\sqrt{n}}} \cdot \bg\right),
 \dots, \psi\left({\frac {g^m}{\sqrt{n}}} \cdot \bg\right)\right)$. Details are given below.

We require a slight refinement of the notion of a ``good'' tuple of vectors from \Cref{sec:halfspace-lb} which now takes into account the lengths of the vectors as well as the angles between them. We say that a specific outcome $(g^1,\dots,g^{3m}) \in (\R^n)^{3m}$ of $(\bg^1,\dots,\bg^{3m}) \sim (N(0,I_n))^{3m}$ is \emph{atypical} if either

\begin{itemize}

\item [(a)] for some $i \in [3m]$ we have ${\frac {\|g^i\|}{\sqrt{n}}} \notin \left[1 - C_1 \sqrt{{\frac {\log n} n}},1 + C_1 \sqrt{{\frac {\log n} n}}\right],$ or

\item [(b)] for some pair $i\neq j$ we have $| {\frac {g^i \cdot g^j}{n}}| > C_1 \sqrt{{\frac {\log n} n}}$.

\end{itemize}
Otherwise we say that $(g^1,\dots,g^m)$ is \emph{typical}.  We defer the proof of the following claim until later:

\begin{claim} \label{claim:typical}
For a suitable choice of the absolute constant $C_1$, we have
$\Pr[(\bg^1,\dots,\bg^{3m})$ is atypical$]\leq 0.005.$
\end{claim}

Hence to show that $(\ref{eq:cheese}) \leq 0.01$ (and finish the proof of \Cref{thm:lb-slab} modulo \Cref{claim:typical}), it suffices to prove the following:

\begin{claim} 
\label{claim:pickwick}
Fix a typical $(g^1,\dots,g^{3m}) \in (\R^n)^{3m}$, where $m = c\sqrt{n}\log n$.
Then for $\bg \sim N(0,I_n)$ we have that
\begin{equation} \label{eq:persuasion}
\dtv\left((\psi(e_1 \cdot \bg),\dots,\psi(e_{3m} \cdot \bg)),
\left(\psi\left({\frac {g^1}{\sqrt{n}}} \cdot \bg\right),
 \dots, \psi\left({\frac {g^{3m}}{\sqrt{n}}} \cdot \bg\right)\right)\right) \leq 0.005.
\end{equation}
\end{claim}
Similar to \Cref{claim:hubert}, we prove \Cref{claim:pickwick} using \Cref{thm:DMR20}.
To apply \Cref{thm:DMR20} we take $\Sigma_1$ to be the identity matrix $I_{3m}$ and $\Sigma_2$ to be the $3m \times 3m$ matrix whose $(i,j)$ entry is ${\frac {g^i \cdot g^j}{n}}$, so a draw from $N(0,\Sigma_1)$ is distributed as $(e_1 \cdot \bg,\dots,e_{3m} \cdot \bg)$ and a draw from $N(0,\Sigma_2)$ is distributed as
$({\frac {g^1}{\sqrt{n}}} \cdot \bg,\dots, {\frac {g^{3m}}{\sqrt{n}}} \cdot \bg).$  Applying the data processing inequality for total variation distance, it follows that the LHS of (\ref{eq:persuasion}) is at most $\dtv(N(0^{3m},\Sigma_1),N(0^{3m},\Sigma_2))$.

Let $A$ denote the matrix $\Sigma_1^{-1}\Sigma_2 - I_{3m}$, so $\lambda_1^2,\dots,\lambda_{3m}^2$ are the eigenvalues of $A^2$  and we have $\sqrt{\lambda_1^2 + \cdots + \lambda_{3m}^2} = \sqrt{\tr(A^2))}.$
By part (a) of the definition of ``typical'' we know that each diagonal entry of $A$ has magnitude at most $3C_1 \sqrt{{\frac {\log n} n}}$, and by part (b) we know that each off-diagonal entry has magnitude at most $C_1 \sqrt{{\frac {\log n} n}}$.
The rest of the proof of \Cref{claim:pickwick} follows the proof of \Cref{claim:hubert} with obvious minor modifications.
%\rnote{Mutatis mutandis, one might say.}
\end{proof}

\medskip

\noindent \emph{Proof of \Cref{claim:typical}.} 
Recalling that $m=c\sqrt{n}/\log n$, a union bound together with \Cref{lem:johnstone} shows that for a suitable choice of $C_1$, part (a) of the ``atypical'' definition holds with probability at most 0.0025. 

For part (b), by a union bound over all ${m \choose 2}$ choices of $i \neq j$ and $m=c\sqrt{n}/\log n$, it is enough to show that for $\bg,\bg'$ independent $N(0,I_n)$ random variables we have
\begin{equation} \label{eq:goalproduct}
\Pr[\bg \cdot \bg' > C_1 \sqrt{n \log n}] < 1/n
\end{equation} (note that we have used the symmetry of the random variable $\bg \cdot \bg'$). By the radial symmetry of the $N(0,I_n)$ distribution we may assume that $\bg =(\br,0,\dots,0)$ where $\br^2 \sim \chi^2_n$, and hence (since $\bg'_1$ is distributed as $N(0,1)$) we have that $\bg \cdot \bg'$ is distributed as $\br \cdot N(0,1)$. By \Cref{lem:johnstone} we have that $\br^2 < 2n$ except with failure probability at most $\exp(-\Theta(n))$, so we may safely assume that $|r| \leq \sqrt{2}n.$ By the standard Gaussian tail bound $\Pr[N(0,1) \geq t] \leq e^{-t^2/2}$ for $t>0$, we see that \Cref{eq:goalproduct} holds for a suitable choice of the absolute constant $C_1$, and \Cref{claim:typical} is proved. \qed










==> sections/lb-slabs.tex <==

%!TEX root = ../distinguishing-writeup.tex

\subsection{A $\tilde{\Omega}(\sqrt{n})$-Sample Lower Bound for Symmetric Convex Bodies (Slabs)} \label{sec:symmetric-lb}

Given a unit vector $v \in \mathbb{S}^{n-1}$ and a positive value $r>0$, we say that the \emph{symmetric slab of width $2r$ in direction $v$} is the symmetric convex set $\Slab_{v,r} := \{x \in \R^n: |v \cdot x| \leq r\}.$  
Our second lower bound shows that $\Omega(\sqrt{n}/\log n)$ samples are needed to distinguish $N(0,I_n)$ from $N(0,I_n)|_K$ where $K$ is an unknown symmetric slab that is promised to have volume roughly $1/2$:
œ
\begin{theorem} \label{thm:lb-slab}
Let $A$ be any algorithm which is given access to samples from an unknown distribution ${\cal D}$ and has the following performance guarantee:

\begin{enumerate}

\item If ${\cal D}=N(0,I_n)$, then with probability at least $9/10$ the algorithm outputs ``un-truncated'';

\item If ${\cal D}=N(0,I_n)|_K$ where $K$ is an unknown symmetric slab with $\vol(K) \in [0.49,0.51]$, then with probability at least $9/10$ the algorithm outputs ``truncated.''

\end{enumerate}
Then $A$ must use at least $\Omega(\sqrt{n}/\log n)$ samples from ${\cal D}$.
\end{theorem}


\begin{proof}
Let $\psi: \R \to \{0,1\}$ be the function $\psi(t) = \Indicator[|t| \leq c]$ where $c \approx 0.68$ is the real number satisfying $\Pr_{\bg \sim N(0,1)}[|\bg| \leq c]=1/2.$
We define a distribution ${\cal K}$ over symmetric slabs as follows: to draw a symmetric slab $\bK \sim {\cal K}$, first draw a standard Normal vector $\bg \sim N(0,I_n)$, and let $\bK=\bK_{\bg}$ be the symmetric slab $\bK = \{x \in \R^n: \psi({\frac {\bg}{\sqrt{n}}} \cdot x)=1\}.$

We observe that given a particular outcome $g$ of $\bg$, the width of the slab $K=\bK_{g}$ is ${\frac {2c \sqrt{n}}{\|g\|}}$, and hence the volume $\vol(K)$ is $\Pr_{\bx \sim N(0,1)}[|\bx| < {\frac {c \sqrt{n}}{\|g\|}}].$ Standard tail bounds on the chi-distribution (which is the distribution of $\|\bg\|$ for $\bg \sim N(0,I_n)$) imply that $\Pr_{\bK \sim {\cal K}}[\vol(\bK) \notin [0.49,0.51]]$ is extremely small, in particular at most $1/n^{\omega(1)}$. 
Hence to prove \Cref{thm:lb-slab}, it suffices to prove an $\Omega(\sqrt{n} / \log n)$ lower bound on the sample complexity of any algorithm $A$ that outputs ``un-truncated'' with probability at least $9/10$ if it is given samples from $N(0,I_n)$ and outputs ``truncated'' with probability at least $91/100$ if it is given samples from $N(0,I_n)|_{\bK}$ where $\bK \sim {\cal K}$. We do this in the rest of the proof.

We consider two different distributions, ${\cal D}_1$ and ${\cal D}_2$, each of which is a distribution over sequences of $m=c\sqrt{n} / \log n$  points in $\R^n$:

\begin{enumerate}

\item A draw of $\overline{\bx}=(\bx^1,\dots,\bx^{m})$ from ${\cal D}_1$  is obtained by having each $\bx^i \in \R^n$ be distributed independently according to $N(0,I_n)$.

\item A draw of $\overline{\bx}=(\bx^1,\dots,\bx^{m})$ from ${\cal D}_2$ is obtained by drawing (once and for all) a set $\bK=\bK_{\bg} \sim {\cal K}$ (so $\bg \sim N(0,I_n)$) and having each $\bx^i$ be distributed independently according to $N(0,I_n)|_{\bK}$, i.e. each $\bx^i$ is drawn from $N(0,I_n)$ conditioned on  satisfying $\psi({\frac {\bg}{\sqrt{n}}} \cdot x)=1.$
\end{enumerate}

We further define two more distributions ${\cal D}'_1$ and ${\cal D}'_2$, each of which is a distribution over sequences of $3m$ points in $\R^n$:

\begin{enumerate}

\item A draw of $\overline{\bx}=(\bx^1,\dots,\bx^{3m})$ from ${\cal D}'_1$ is obtained as follows: $\bx^i$ is taken to be $\bb_i \bg^i$ where each $\bb_i$ is an independent uniform draw from $\zo$ and each $\bg^i$ is an independent draw from $N(0,I_n)$.

\item A draw of $\overline{\bz}=(\bz^1,\dots,\bz^{3m})$ from ${\cal D}'_2$ is obtained as follows:  once and for all draw $\bg \sim N(0,I_n)$, and take $\bz^i$ to be $\bg^i \cdot \psi({\frac {\bg}{\sqrt{n}}} \cdot \bg^i)$ where each $\bg^i$ is an independent draw from $N(0,I_n)$.

\end{enumerate}


Suppose that algorithm $A$ successfully distinguishes between ${\cal D}_1$ and ${\cal D}_2$, i.e. it outputs ``un-truncated'' with probability at least 9/10 when run on a draw from ${\cal D}_1$ and outputs ``truncated'' with probability at least 91/100 when run on a draw from ${\cal D}_2.$
We claim that then there is an algorithm $A'$ which successfully distinguishes between ${\cal D}'_1$ and ${\cal D}'_2$, i.e. it outputs ``un-truncated'' with probability at least 89/100 when run on a draw from ${\cal D}'_1$ (recall that this is a sequence of $3m$ points in $\R^n$) and outputs ``truncated'' with probability at least 90/100 when run on a draw from ${\cal D}'_2.$  This algorithm $A'$ simply takes the first $m$ nonzero points in its $3m$-point input sequence and uses them as input to $A$.  (We may suppose that $A'$ fails if there are fewer than $m$ nonzero points in the $3m$-point sample; it is easy to see that whether the input to $A'$ is drawn from ${\cal D}'_1$ or ${\cal D}'_2$, the probability of failure is at most $1/n^{\omega(1)}$ and hence is negligible.)  If the input sequence is a draw from ${\cal D}'_1$ then the input that $A'$ gives to $A$ is distributed according to ${\cal D}_1$, and if the input is a draw from ${\cal D}'_2$ then the input sequence that $A'$ gives to $A$ is distributed according to ${\cal D}_2$ (note that we may safely ignore the probability-0 event that some $\bg^i$ drawn from $N(0,I_n)$ is the zero vector).

Given the above claim, to prove \Cref{thm:lb-slab} it suffices to show that any algorithm $A'$ with the performance guarantee described above must have $3m = \Omega(\sqrt{n}/\log n).$  This follows from the statement
\begin{equation}
\label{eq:dtvprimes}
\text{If $m = c \sqrt{n}/\log n$, then~~~~}\dtv({\cal D}'_1,{\cal D}'_2) \leq 0.01.
\end{equation}
The rest of the proof establishes (\ref{eq:dtvprimes}).

Consider a coupling of the two distributions ${\cal D}'_1$ and ${\cal D}'_2$ as follows. A draw from the joint coupled distribution of $({\cal D}'_1,{\cal D}'_2)$ is generated in the following way:

\begin{itemize}

\item Let $(\bb_1,\dots,\bb_{3m})$ be a uniform random string from $\zo^{3m}$. 
\item Let $\bg, \bg^1,\dots,\bg^m$ be $3m+1$ independent draws from $N(0,I_n).$
\item The draw from the joint coupled distribution is $(\overline{\bx},\overline{\bz})$ where
\[
\text{for each $i =1,\dots,3m$,~~~}\bx^i = \bb_i \bg^i \quad \text{and}\quad
 \bz^i=\psi\left({\frac {\bg}{\sqrt{n}}} \cdot \bg^i\right) \bg^i .
\]
\end{itemize}
It is easily verified that this is indeed a valid coupling of ${\cal D}'_1$ and ${\cal D}'_2$.
Writing $\overline{\bg}$ to denote $(\bg^1,\dots,\bg^m)$, by the same reasoning as in \Cref{eq:gourd} and \Cref{eq:pumpkin}, we have that
\begin{align}
\dtv({\cal D}'_1,{\cal D}'_2) 
&= \dtv((\bx^1,\dots,\bx^{3m}),(\bz^1,\dots,\bz^{3m})) \nonumber\\
&=\dtv\left((\bb_1\bg^1,\dots,\bb_{3m}\bg^{3m}),
\left(
\psi\left({\frac {\bg}{\sqrt{n}}} \cdot \bg^1\right) \bg^1,
\psi\left({\frac {\bg}{\sqrt{n}}} \cdot \bg^{3m}\right) \bg^{3m}
 \right)\right) \nonumber\\
 &\leq \Ex_{\overline{\bg}} \left[\dtv\left((\bb_1\bg^1,\dots,\bb_{3m}\bg^{3m}),
\left(
\psi\left({\frac {\bg}{\sqrt{n}}} \cdot \bg^1\right) \bg^1,
\psi\left({\frac {\bg}{\sqrt{n}}} \cdot \bg^{3m}\right) \bg^{3m}
 \right)\right)\right] \nonumber\\
 &\leq \Ex_{\overline{\bg}}\left[\dtv\left((\bb_1,\dots,\bb_{3m}),\left(\psi\left({\frac {\bg}{\sqrt{n}}} \cdot \bg^1\right),
 \dots, \psi\left({\frac {\bg}{\sqrt{n}}} \cdot \bg^{3m}\right)\right)\right)\right] \label{eq:ham}
\end{align}
It remains to show that if $m = c \sqrt{n}/\log n$ then $(\ref{eq:ham}) \leq 0.01.$

We observe that for $\bg \sim N(0,I_n)$, we have that $\Pr[\psi(e_i \cdot \bg)=1]=\Pr[\psi(\bg_i)=1]=1/2$. Since the random variables $\{\bg_i\}_{i=1,\dots,3m}$ are independent, we have that the joint distribution of $(\bb_1,\dots,\bb_{3m})$ is identical to the joint distribution of $(\psi(e_1 \cdot \bg),\dots,\psi(e_{3m} \cdot \bg))$, namely, both distributions are uniform over $\zo^{3m}.$ Thus we have that
\begin{equation}
\label{eq:cheese}
(\ref{eq:ham}) = \Ex_{\overline{\bg}}\left[\dtv\left((\psi(e_1 \cdot \bg),\dots,\psi(e_{3m} \cdot \bg)),
\left(\psi\left({\frac {\bg^1}{\sqrt{n}}} \cdot \bg\right),
 \dots, \psi\left({\frac {\bg^{3m}}{\sqrt{n}}} \cdot \bg\right)\right)\right)\right].
 \end{equation}
The rest of the argument proceeds similarly to the proof of \Cref{claim:dtvhalfspace} following (\ref{eq:humphrey}): briefly, for most outcomes $(g^1,\dots,g^{3m})$ of $\bg^1,\dots,\bg^{3m}$, the covariance structure of the two $3m$-dimensional Gaussians $(e_1 \cdot \bg,\dots,e_{3m} \cdot \bg)$ and $({\frac {g^1}{\sqrt{n}}} \cdot \bg,\dots,{\frac {g^{3m}}{\sqrt{n}}} \cdot \bg)$ are similar enough that we can bound the variation distance between those two Gaussians, which implies a bound on the variation distance between $(\psi(e_1 \cdot \bg),\dots,\psi(e_{3m} \cdot \bg))$ and $\left(\psi\left({\frac {g^1}{\sqrt{n}}} \cdot \bg\right),
 \dots, \psi\left({\frac {g^m}{\sqrt{n}}} \cdot \bg\right)\right)$. Details are given below.

We require a slight refinement of the notion of a ``good'' tuple of vectors from \Cref{sec:halfspace-lb} which now takes into account the lengths of the vectors as well as the angles between them. We say that a specific outcome $(g^1,\dots,g^{3m}) \in (\R^n)^{3m}$ of $(\bg^1,\dots,\bg^{3m}) \sim (N(0,I_n))^{3m}$ is \emph{atypical} if either

\begin{itemize}

\item [(a)] for some $i \in [3m]$ we have ${\frac {\|g^i\|}{\sqrt{n}}} \notin \left[1 - C_1 \sqrt{{\frac {\log n} n}},1 + C_1 \sqrt{{\frac {\log n} n}}\right],$ or

\item [(b)] for some pair $i\neq j$ we have $| {\frac {g^i \cdot g^j}{n}}| > C_1 \sqrt{{\frac {\log n} n}}$.

\end{itemize}
Otherwise we say that $(g^1,\dots,g^m)$ is \emph{typical}.  We defer the proof of the following claim until later:

\begin{claim} \label{claim:typical}
For a suitable choice of the absolute constant $C_1$, we have
$\Pr[(\bg^1,\dots,\bg^{3m})$ is atypical$]\leq 0.005.$
\end{claim}

Hence to show that $(\ref{eq:cheese}) \leq 0.01$ (and finish the proof of \Cref{thm:lb-slab} modulo \Cref{claim:typical}), it suffices to prove the following:

\begin{claim} 
\label{claim:pickwick}
Fix a typical $(g^1,\dots,g^{3m}) \in (\R^n)^{3m}$, where $m = c\sqrt{n}\log n$.
Then for $\bg \sim N(0,I_n)$ we have that
\begin{equation} \label{eq:persuasion}
\dtv\left((\psi(e_1 \cdot \bg),\dots,\psi(e_{3m} \cdot \bg)),
\left(\psi\left({\frac {g^1}{\sqrt{n}}} \cdot \bg\right),
 \dots, \psi\left({\frac {g^{3m}}{\sqrt{n}}} \cdot \bg\right)\right)\right) \leq 0.005.
\end{equation}
\end{claim}
Similar to \Cref{claim:hubert}, we prove \Cref{claim:pickwick} using \Cref{thm:DMR20}.
To apply \Cref{thm:DMR20} we take $\Sigma_1$ to be the identity matrix $I_{3m}$ and $\Sigma_2$ to be the $3m \times 3m$ matrix whose $(i,j)$ entry is ${\frac {g^i \cdot g^j}{n}}$, so a draw from $N(0,\Sigma_1)$ is distributed as $(e_1 \cdot \bg,\dots,e_{3m} \cdot \bg)$ and a draw from $N(0,\Sigma_2)$ is distributed as
$({\frac {g^1}{\sqrt{n}}} \cdot \bg,\dots, {\frac {g^{3m}}{\sqrt{n}}} \cdot \bg).$  Applying the data processing inequality for total variation distance, it follows that the LHS of (\ref{eq:persuasion}) is at most $\dtv(N(0^{3m},\Sigma_1),N(0^{3m},\Sigma_2))$.

Let $A$ denote the matrix $\Sigma_1^{-1}\Sigma_2 - I_{3m}$, so $\lambda_1^2,\dots,\lambda_{3m}^2$ are the eigenvalues of $A^2$  and we have $\sqrt{\lambda_1^2 + \cdots + \lambda_{3m}^2} = \sqrt{\tr(A^2))}.$
By part (a) of the definition of ``typical'' we know that each diagonal entry of $A$ has magnitude at most $3C_1 \sqrt{{\frac {\log n} n}}$, and by part (b) we know that each off-diagonal entry has magnitude at most $C_1 \sqrt{{\frac {\log n} n}}$.
The rest of the proof of \Cref{claim:pickwick} follows the proof of \Cref{claim:hubert} with obvious minor modifications.
%\rnote{Mutatis mutandis, one might say.}
\end{proof}

\medskip

\noindent \emph{Proof of \Cref{claim:typical}.} 
Recalling that $m=c\sqrt{n}/\log n$, a union bound together with \Cref{lem:johnstone} shows that for a suitable choice of $C_1$, part (a) of the ``atypical'' definition holds with probability at most 0.0025. 

For part (b), by a union bound over all ${m \choose 2}$ choices of $i \neq j$ and $m=c\sqrt{n}/\log n$, it is enough to show that for $\bg,\bg'$ independent $N(0,I_n)$ random variables we have
\begin{equation} \label{eq:goalproduct}
\Pr[\bg \cdot \bg' > C_1 \sqrt{n \log n}] < 1/n
\end{equation} (note that we have used the symmetry of the random variable $\bg \cdot \bg'$). By the radial symmetry of the $N(0,I_n)$ distribution we may assume that $\bg =(\br,0,\dots,0)$ where $\br^2 \sim \chi^2_n$, and hence (since $\bg'_1$ is distributed as $N(0,1)$) we have that $\bg \cdot \bg'$ is distributed as $\br \cdot N(0,1)$. By \Cref{lem:johnstone} we have that $\br^2 < 2n$ except with failure probability at most $\exp(-\Theta(n))$, so we may safely assume that $|r| \leq \sqrt{2}n.$ By the standard Gaussian tail bound $\Pr[N(0,1) \geq t] \leq e^{-t^2/2}$ for $t>0$, we see that \Cref{eq:goalproduct} holds for a suitable choice of the absolute constant $C_1$, and \Cref{claim:typical} is proved. \qed










==> sections/lower-bounds.tex <==
%!TEX root = ../distinguishing-writeup.tex
%\newpage

\section{Lower Bounds}
\label{sec:lbs}

In \Cref{sec:halfspace-lb}, we present a $\wt{\Omega}(\sqrt{n})$ lower-bound for distinguishing Gaussians truncated to LTFs, followed by a $\wt{\Omega}(n)$ lower bound for distinguishing Gaussians truncated to symmetric convex sets in \Cref{sec:symmetric-lb}. (The specific symmetric convex set we use for the latter is the slab.) Finally, in \Cref{sec:mix-lb}, we present a $\Omega(n)$ lower bound for distinguishing a mixture of Gaussians truncated to symmetric convex sets. 

\input{sections/lb-halfspaces}
\input{sections/lb-slabs}
\input{sections/lb-mixtures}


==> sections/wishart-lb.tex <==
%!TEX root = ../distinguishing-writeup.tex

\newcommand{\z}{{\bz}}

\section{An $\Omega(n)$-Sample Lower Bound for Testing Truncation}
\label{sec:wishart-lb}

In this section, we present an $\Omega(n)$-sample lower bound for testing convex truncation. Our lower bound is information-theoretic and applies to all algorithms, computationally efficient or otherwise. More formally, we prove the following:

\begin{theorem} \label{thm:chi-lb}
Let $A$ be any algorithm which is given access to samples from an unknown distribution ${\cal D}$ and has the following performance guarantee:
\begin{enumerate}
\item If ${\cal D}=N(0,I_n)$, then with probability at least $9/10$ the algorithm outputs ``un-truncated'';
\item If ${\cal D} \in \Psymm$ and has $\dtv({\cal D},N(0,I_n))=1$ then with probability at least $9/10$ the algorithm outputs ``truncated.''\footnote{We note that if ${\cal D} \in \Psymm$ has $\dtv({\cal D},N(0,I_n))=1$, then $\calD$ is obtained by conditioning the Gaussian distribution $N(0,I_n)$ on a symmetric convex set of zero measure. In order for this to be a well-defined operation (see for e.g. \cite{BorelKolmogorov:wikipedia}), we need to specify a suitable limiting sequence of sets of positive measure; we defer this discussion to \Cref{rem:reassurance}.}
\end{enumerate}
Then $A$ must use at least $\Omega(n)$ samples from ${\cal D}$.
\end{theorem}

As $\Psymm \sse \Pconv$ and $\Psymm \sse \Mix$, \Cref{thm:chi-lb} immediately that the algorithms~\Convex~and \symmconvex~are optimal in terms of sample complexity for testing convex truncation and truncation by a mixture of symmetric convex sets respectively.

\subsection{Useful Preliminaries}
\label{subsec:wishart-prelims}

Before proceeding to the proof of \Cref{thm:chi-lb}, we introduce some useful notation and recall preliminaries on the \emph{Wishart distribution}. Let $\mathfrak{C}_p$ denote the cone of $p\times p$ positive semi-definite matrices. We will write $(x)_+ := \max(0,x)$.

\begin{definition}[Wishart distribution] \label{def:wishart}
	For $p\leq n$, let \emph{$\Wis(p,n)$} denote the \emph{Wishart distribution on $p\times p$ matrices with $n$ degrees of freedom}, i.e. the distribution on symmetric positive-semidefinite matrices obtained by
	\begin{enumerate}
		\item Drawing $\bG_i \sim N(0, I_p)$ for $i \in [n]$.
		\item Outputting $\bS := \sumi \bG_i \bG_i^{T}$.
	\end{enumerate} 
\end{definition}

We will make use of the following well-known expression for the density of $\Wis(p,n)$.

\begin{fact}[see e.g.~\cite{eaton2007wishart}] \label{fact:wishart-density}
	Let $\Psi_{p,n}$ denote the density of $\Wis(p,n)$. We have
\begin{equation} \label{eq:wis-density}
	\Psi_{p,n}(A) = \frac{\det(A)^{(n-p-1)/2}\cdot \exp\pbra{-\mathrm{Tr}(A)/2}}{2^{np/2}\pi^{p(p-1)/4}\prod_{i=1}^p \Gamma\pbra{\frac{1}{2}(n + 1-i)}} \cdot \mathbf{1}\cbra{A \succeq 0}.
\end{equation}
\end{fact}

We will also require the following central limit theorem for the log-determinant of a matrix drawn according to the Wishart distribution $\Wis(p,n)$ when $p = \Theta(n)$. The following statement was obtained by Jonsson~\cite{JONSSON19821}.

\begin{theorem}[Theorem~5.1 of~\cite{JONSSON19821}] \label{thm:dagman}
	Suppose $n, p = p(n) \in \N$ are such that 
	\[\lim_{n\to\infty} \frac{p}{n} = y \in (0,1).\]
	Then as $n\to\infty$, the following holds:
	\[\frac{1}{\sqrt{-2\log(1-y)}}\log\pbra{\frac{\det(\bW)}{(n-1)\cdots(n-p)}} \longrightarrow_L ~N(0,1) \qquad\text{for~}\bW\sim\Wis(p,n),\] 
	where the convergence is in distribution.
\end{theorem}


\subsection{Proof of \Cref{thm:chi-lb}}
\label{subsec:wishart-lb-pf}

We start by formally defining our distribution over truncations of $N(0,I_n)$ by symmetric convex sets. 

\begin{notation}
	Let $\calD_{\mathrm{plane}}$ be the distribution on origin-centered hyperplanes induced by the Haar measure on $\S^{n-1}$, i.e. it is the distribution on hyperplanes obtained by
	\begin{enumerate}
		\item First drawing a Haar-random vector $\bv\sim \S^{n-1}$; and then
		\item Outputting the origin-centered hyperplane $\bv^\perp := \cbra{ x \in\R^n: \abra{x, \bv} = 0}$.
	\end{enumerate}
\end{notation}

In what follows, we will show that no algorithm can distinguish between $N(0,I_n)$ and $N(0, I_n)\mid_{\bK}$ for $\bK\sim\Dslab$ with $cn$ samples for some sufficiently small absolute constant $c$; note that this immediately implies \Cref{thm:chi-lb}. We first show that distinguishing between $N(0,I_n)$ and $N(0, I_n)|_{\bK}$  is equivalent to distinguishing between Wishart distributions with $n$ and $(n-1)$ degrees of freedom.

\begin{remark} \label{rem:reassurance} 
The attentive reader may notice that the sets $\bK$ defined above have
$\vol(\bK)=0$, and thus $N(0,I_n)|_{\bK}$ is the standard normal distribution conditioned on an event of measure zero.
For this to be a well defined operation (see e.g. \cite{BorelKolmogorov:wikipedia}),  we need to specify how our measure-zero sets are obtained as the limit of a sequence of sets of positive measure.
The limiting process we use for a set $K = \bv^\perp$ is taking a sequence of slabs 
\[
\bv^{\perp}_\epsilon := \{x: |v \cdot x| \leq \eps\}
\]
and letting $\eps \to 0$. In the limit, the distribution induced for $N(0,I_n)|_{\bK}$ is a symmetric distribution restricted to $\bK$ corresponding to $N(0, I_{n-1})$.
\end{remark}

\begin{claim} \label{claim:reduction-to-wishart}
For $p\leq n-1$, there exists an algorithm $\calA$ which can distinguish between $N(0,I_n)$ and $N(0, I_n)|_{\bK}$ where $\bK\sim\Dslab$ (i.e. outputs ``un-truncated'' with probability $9/10$ given samples from the former and outputs ``truncated'' with probability $9/10$ given samples from the latter)  
with $p$ samples 
{if and only if} 
there exists an algorithm $\calA'$ that can distinguish between $\Wis(p,n)$ and $\Wis(p, n-1)$
with $1$ sample. 
\end{claim}

\begin{proof}
We start with the ``if" direction---namely, 
the existence of $\calA'$ immediately allows us to distinguish between $N(0,I_n)$ and $N(0,I_n)|_{\bK}$ given $p$ samples $\x{1},\ldots, \x{p}$ by computing the $p\times p$ matrix $\bW$ given by 
	\begin{equation} \label{eq:ip-constraints}
		\bW_{i,j} := \abra{\x{i},\x{j}}.
	\end{equation}
	Note that if $\x{i} \sim N(0,I_n)$ for $i\in[p]$, then $\bW \sim \Wis(p,n)$. On the other hand, if $\x{i} \sim N(0,I_n)|_{\bK}$ for $i\in[p]$, then since the distribution of the inner product of two draws from $N(0,I_{n})|_{K}$ is the same for all $(n-1)$-dimensional origin-centered hyperplanes $K$, it is easy to see that $\bW \sim \Wis(p,n-1)$. 
	
	
Before proceeding with the proof for the ``only if" direction, i.e., how the existence of $\calA$ implies the existence of $\calA'$, we make a few important observations. 	
	
First, observe that any $p\times p$ matrix $W$ where
	\[W_{i,j} = \abra{x^{(i)},x^{(j)}} \qquad\text{where~} x^{(i)},x^{(j)}\in\R^n\]
	uniquely determines the collection of points $\{x^{(1)}, \ldots, x^{(p)}\}$ up to an orthogonal transformation. 
	
	
Given any symmetric $p\times p$ psd matrix $W$, we define $\Sigma(W)$ as 	
%	This is immediate from the uniqueness (up to orthogonal transformations) of the realization of vectors given a Gram matrix.
	%Turning to the reverse direction, given a symmetric , we
	%denote 
	\[\Sigma(W) := \cbra{\pbra{x^{(1)},\ldots, x^{(p)}} \in \R^{np}: W_{i,j} = \abra{x^{(i)}, x^{(j)}}}.\]
	Note that $\Sigma(W)$ is a compact Hausdorff set (under the usual topology on $\R^{np}$). As the orthogonal group $\mathrm{O}(n)$ acts transitively on $\Sigma(W)$ for all symmetric $p\times p$ matrices $W$---where the group action is given by the map 
	\[
	\pbra{Q, ({x^{(1)},\ldots, x^{(p)}})} \mapsto \pbra{Qx^{(1)},\ldots, Qx^{(p)}}
	\]
	for $Q \in \mathrm{O}(n)$---it follows by Weil's theorem (cf.~Theorem~6.2 of~\cite{diestel2014joys}) that there is a unique $\mathrm{O}(n)$-invariant probability measure on $\Sigma(W)$. Call this probability measure ${\cal D}_{\Sigma(W)}$. 
	
	Given matrix $W\in\mathfrak{C}_p$, consider the process that 
	(a) computes a canonical choice of $p$ points $(x^{(1)},\ldots,x^{(p)})\in \Sigma(W)$; and then (b) applies a Haar-random orthogonal transformation $\bQ \sim \mathrm{O}(n)$ to output the points 
	\[\bQ(W) := ({\bQ x^{(1)},\ldots, \bQ x^{(p)}}).\]
Given any $W\in\mathfrak{C}_p$, the distribution of $\bQ(W)$ on $\Sigma(W)$ is $\mathrm{O}(n)$-invariant under the above group action. Furthermore, by the preceding discussion, this is the unique such measure on $\Sigma(W)$, ${\cal D}_{\Sigma(W)}$.  We record this fact below. 
\begin{fact}~\label{fact:invariant-measure}
For every matrix $W\in\mathfrak{C}_p$, there is a unique $\mathrm{O}(n)$-invariant probability measure ${\cal D}_{\Sigma(W)}$ on the set $\Sigma(W)$, and further, the algorithm given by (a) and (b) above samples from ${\cal D}_{\Sigma(W)}$. 
\end{fact}


The next claim states that  samples in the un-truncated case can be simulated by sampling  $\bW\sim\Wis(p,n)$ and then sampling from ${\cal D}_{\Sigma(\bW)}$.  
\begin{claim}~\label{clm:simulation-untruncated}
For $p<n$, the distribution of $(\x{1}, \ldots, \x{p})$ where each $\x{i} \sim N(0,I_n)$
is the same as  sampling $\bW\sim\Wis(p,n)$ and then sampling $(\z^{(1)}, \ldots, \z^{(p)}) \sim {\cal D}_{\Sigma(\bW)}$. 
\end{claim}
\begin{proof}
Consider a sample $(\x{1}, \ldots, \x{p})$ where each $\x{i} \sim N(0,I_n)$. Corresponding to this draw, we define  $\bW$ given by \Cref{eq:ip-constraints}. Note that the distribution of $\bW$ is given by $\Wis(p,n)$. Thus, the distribution of $(\x{1}, \ldots, \x{p})$ can be equivalently defined as sampling $\bW \sim \Wis(p,n)$ and then sampling from the distribution
$(\x{1}, \ldots, \x{p}) \sim N(0,I_n)^p$ conditioned on the Gram matrix of $(\x{1},\dots,\x{p})$ being $\Sigma(\bW)$ (we denote this conditional distribution by ${\cal X}_{\bW}$).

The crucial observation is that the distribution of $(\x{1}, \ldots, \x{p})$ is $\mathrm{O}(n)$-invariant. Since the image of $\Sigma(W)$ (for any $W$) under $\mathrm{O}(n)$ is $\Sigma(W)$ itself, it follows that for every $W$, the conditional distributions ${\cal X}_{W}$ are $\mathrm{O}(n)$-invariant. By applying \Cref{fact:invariant-measure}, it follows that for every $W$, ${\cal X}_W$ is the same as ${\cal D}_{\Sigma(W)}$, thus finishing the proof. 
\end{proof} 

We now have the analogous claim for the truncated case as well. 
\begin{claim}\label{clm:simulation-truncated}
For $p<n$, the distribution of $(\x{1}, \ldots, \x{p})$ where each $\x{i} \sim N(0, I_n)|_{\bK}$ where $\bK\sim\Dslab$
is the same as  sampling $\bW\sim\Wis(p,n-1)$ and then sampling $(\z^{(1)}, \ldots, \z^{(p)}) \sim {\cal D}_{\Sigma(\bW)}$. 
\end{claim} 
\begin{proof}
Note that in this case as well, the distribution $(\x{1}, \ldots, \x{p})$ is invariant under the action of $\mathrm{O}(n)$. With this observation, the proof in this case is identical to that of \Cref{clm:simulation-untruncated} except that the matrix $\bW$ given by  \Cref{eq:ip-constraints} is now distributed as $\Wis(p,n-1)$.
\end{proof}

Thus, now consider the process where given $\bW$, we output $(\z^{(1)}, \ldots, \z^{(p)}) \sim {\cal D}_{\Sigma(W)}$. We observe that 
\begin{enumerate}
\item If $\bW \sim \Wis(p,n)$, then $(\z^{(1)}, \ldots, \z^{(p)})$ are distributed as $p$ i.i.d.~samples from  $N(0,I_n)$. 
\item If $\bW \sim \Wis(p,n-1)$, then $(\z^{(1)}, \ldots, \z^{(p)})$ are distributed as $p$ i.i.d.~samples from   $N(0, I_n)|_{\bK}$ where $\bK\sim\Dslab$.
\end{enumerate}

Thus, an algorithm $\calA$ which can distinguish $N(0,I_n)$ versus $N(0, I_n)|_{\bK}$ (where $\bK\sim\Dslab$) with $p$ samples can distinguish between $\Wis(p,n)$ and $\Wis(p,n-1)$ with one sample (with the same distinguishing probability). 
\end{proof}

With this in hand, \Cref{thm:chi-lb} is immediately implied by the following:
\begin{equation} \label{eq:new-tv-goal}
	\dtv\pbra{\Wis(p, n), \Wis(p, n-1)} \leq 0.1 \qquad\text{for~} p = 0.00001(n-1).
\end{equation}
The rest of the proof establishes \Cref{eq:new-tv-goal} for the above choice of $p$. Writing $\mu_{p, n-1}$ for the measure on $\mathfrak{C}_p$ corresponding to the density $\Psi_{p,n-1}$, we have 
\begin{equation} \label{eq:tv-dist-1}
	\dtv\pbra{\Wis(p, n), \Wis(p, n-1)} = \int_{\mathfrak{C}_p} \pbra{1 - \frac{\Psi_{p,n}(A)}{\Psi_{p, n-1}(A)}}_{+} \,d\mu_{p, n-1}(A).
\end{equation}
For notational convenience, we define 
\[
\alpha_{p,n}(A) := {\log\pbra{\frac{\Psi_{p,n}(A)}{\Psi_{p,n-1}(A)}}}.
\]
Note that in order to establish \Cref{eq:new-tv-goal}, it suffices to show that 
\begin{equation} \label{eq:final-goal}
	\abs{\alpha_{p,n}(A)} \leq 0.02 \text{~with probability at least~} 0.99\text{~under~}\mu_{n-1}.
\end{equation}
To see this, note that $0\leq \pbra{1 - \frac{\Psi_n(A)}{\Psi_{n-1}(A)}}_+ \leq 1$ for all $A$, and so using \Cref{eq:tv-dist-1} we have 
\begin{itemize}
	\item A contribution of at most $0.01$ to the variation distance from outcomes of $A$ such that $|\alpha_{p,n}(A)| > 0.02$; and 
	\item A contribution of at most $1-\exp\pbra{-0.02} \leq 0.04$ to the variation distance from outcomes of $A$ such that $|\alpha_{p,n}(A)|\leq 0.02$.  
\end{itemize}
Using \Cref{fact:wishart-density}, for $A \in \mathfrak{C}_p$ we can write 
\begin{align}
	\alpha_{p,n}(A) &= \log\bigg(\frac{\det(A)^{1/2}}{2^{p/2}}\cdot\frac{\Gamma\pbra{(n-p)/{2}}}{\Gamma\pbra{{n}/{2}}}\bigg) \nonumber\\
	&= \frac{\log\det(A)- p}{2} - \sum_{i= \frac{n-p}{2}}^{\frac{n-2}{2}} \log i \nonumber\\ 
	&= \frac{\log\det(A)- p}{2} - \sum_{i=1}^{\frac{p}{2}} \log\pbra{\frac{n-p}{2} + i - 1} \nonumber\\
	&= \frac{\log\det(A)- p}{2} - \pbra{\sum_{i=1}^{\frac{p}{2}} \log\pbra{n-p +2(i-1)}} + \frac{p}{2} \nonumber\\
	&= \frac{\log\det(A)}{2} - {\sum_{i=1}^{\frac{p}{2}} \log\pbra{n-p +2(i-1)}}. \label{eq:simplified-alpha}
\end{align}

We pause to recall \Cref{thm:dagman}, from which we know that the $\log\det(\bW)$ where $\bW\sim\Wis(n-1,p)$ converges in distribution to a $N(\mu,\sigma^2)$ random variable where 
\[\mu := \sum_{j=1}^p \log\pbra{n - p + (j-2)}\qquad\text{and}\qquad \sigma^2 := 2\log\pbra{\frac{1}{1-p/(n-1)}} = 2\log\pbra{\frac{1}{0.99999}}.\]
%In particular, this implies that for all $t\in\R$, there exists a large enough $n$ such that 
%\[\mathrm{d}_{\mathrm{CDF}}\pbra{\log\det(\bW), N(\mu,\sigma^2)} \leq 0.005.\]
This in turn implies that for every $t\in \R$, there exists $n$ large enough such that
\begin{equation} \label{eq:clt-wishart-app}
	\Prx_{\bW\sim\Wis(p,n-1)}\sbra{\abs{\log\det(\bW) - \mu} > t} \leq 0.005 + \Prx_{\bg\sim N(0,\sigma^2)}\sbra{|\bg| > t}.
\end{equation}

Returning to \Cref{eq:simplified-alpha}, we can write
\begin{align*}
	\alpha_{p,n}(A) &= \frac{\log\det(A) - \mu}{2} + \frac{\mu - 2{\sum_{i=1}^{\frac{p}{2}} \log\pbra{n-p +2(i-1)}}}{2}\\
	&= \frac{\log\det(A) - \mu}{2} + \frac{1}{2}\pbra{\sum_{j=1}^p \log(n-p + (j-2))  - 2\sum_{i=1}^{\frac{p}{2}} \log(n-p+2(i-1))}\\
	&= \frac{\log\det(A) - \mu}{2} + \frac{1}{2}\sum_{i=1}^{p/2}\log\pbra{\frac{n-p + 2j-1}{n-p + 2j-2}}\\
%	&= \frac{\log\det(A) - \mu}{2} + \frac{1}{2}\sum_{i=1}^{p/2}\log\pbra{1 + \frac{1}{n-p + 2j-2}}\\
	&\leq \frac{\log\det(A) - \mu}{2} + \frac{p}{4}\log\pbra{1 + \frac{1}{n-p}}\\
	&\leq \frac{\log\det(A) - \mu}{2} + 0.001
\end{align*}
where the final inequality uses the fact that $1 + x\leq e^x$ and our choice of $p = 0.00001n$. Combining this with \Cref{eq:clt-wishart-app}, we have that for sufficiently large $n$ (where we take $t = 0.038$),
\begin{align*}
	\Prx_{\bW\sim\Wis(p,n-1)}\sbra{|\alpha_{p,n}(\bW)| > 0.02} 
	&\leq \Prx_{\bW\sim\Wis(p,n-1)}\sbra{\abs{\log\det(\bW) - \mu} > 0.038}\\
	&\leq 0.005 + \Prx_{\bg\sim N(0,\sigma^2)}\sbra{|\bg| > 0.038}\\
	&\leq 0.01,
\end{align*} 
establishing \Cref{eq:final-goal}. This in turn establishes \Cref{eq:tv-dist-1}, which together with \Cref{claim:reduction-to-wishart} completes the proof of \Cref{thm:chi-lb}. \qed 

